Priority Coordination Games: Hodge Decomposition and a Sharp Design Limit

In decentralised priority coordination, agents announce priority levels and a shared resource serves them in decreasing order, as at an unsignalised intersection; the levels form the decision layer of a hierarchical controller. Such interactions are routinely replaced by a potential game, i.e.\ by a common objective, for analysis and design. This paper determines what that surrogate misses, using the Hodge decomposition of the incentives into a potential component, which a common objective can represent, and a harmonic component, which it cannot. For the linear payoff, both components are obtained in closed form on every conflict graph and for every deterministic tie-breaking protocol: in common units, the harmonic energy is the number of conflicts and the potential energy adds the number of adjacent pairs of conflicts. Consequently, for every rationality parameter, the best common-objective model of the agents' choice log-odds, weighted uniformly over unilateral moves, has a relative squared error of at least $1/(d_{\max}+1)$, where $d_{\max}$ is the largest number of conflicts of one agent; for an eight-vehicle intersection it is exactly one fifth, for any number of priority levels. Invisible to strict-improvement dynamics, the missed component is, under low-rationality log-linear learning with uniform revision and to leading order, the stationary probability current, and its energy sets the entropy-production rate. Payoff design cannot remove it: on the complete conflict graph of $N$ agents, under a total-order protocol and with at least three priority levels, every nonconstant rank-based payoff leaves a relative error of at least $1/N$, with equality exactly for affine payoffs.

==> figs/backup/SMV3.tex <==
% ---------------------------------------------------------------
% Supplementary material. Typeset with the main text (one compile,
% no xr/aux); split the PDF at this page for submission.
% ---------------------------------------------------------------
\clearpage
\onecolumn
\setcounter{page}{1}
\renewcommand{\thesection}{\Alph{section}}\setcounter{section}{0}
\renewcommand{\thesubsection}{\thesection.\arabic{subsection}}
\renewcommand{\theequation}{S\arabic{equation}}\setcounter{equation}{0}
\renewcommand{\thetable}{S\arabic{table}}\setcounter{table}{0}
\renewcommand{\thefigure}{S\arabic{figure}}\setcounter{figure}{0}\renewcommand{\theHfigure}{S\arabic{figure}}
\renewcommand{\theHsection}{S\Alph{section}}\renewcommand{\theHsubsection}{S\Alph{section}.\arabic{subsection}}
\renewcommand{\theHequation}{S\arabic{equation}}\renewcommand{\theHtable}{S\arabic{table}}
% steps of the proof of Theorem~\ref{thm:finiteK}: numbered by a counter, referenced by label
\newcounter{pstep}\setcounter{pstep}{-1}
\makeatletter
\newcommand{\stepsection}[2]{\stepcounter{pstep}\subsection{Step~\thepstep: #2}\edef\@currentlabel{\thepstep}\label{step:#1}}
\makeatother
\markboth{\hskip25pc SUPPLEMENTARY MATERIAL}{Lin \MakeLowercase{\textit{et al.}}: Supplementary material}
\begin{center}
{\Large\bfseries Supplementary Material for}\\[4pt]
{\large\itshape How Far Is Priority Coordination from a Potential Game?\\ Hodge Decomposition and Sharp Bound}\\[10pt]
\end{center}
\bigskip
\noindent
This document contains complete proofs of the results whose proofs are omitted or only sketched in the main text, and
documents the computer-assisted steps. References of the form ``Theorem~\ref{thm:finiteK}'' or
``\eqref{eq:SOS}'' point to the main text; auxiliary results proved here are numbered S1, S2, \dots, and equations
(S1), (S2), \dots. Appendix~\ref{app:finiteK} comes first because it proves the main technical result,
Theorem~\ref{thm:finiteK}; Theorem~\ref{thm:spectrum} is proved in Appendix~\ref{sec:cont}, which uses one lemma of
Appendix~\ref{app:finiteK}.
\begin{itemize}
\item Appendix~\ref{app:finiteK} proves Theorem~\ref{thm:finiteK}
(finite quantisation), in fourteen steps following the five-part
architecture of Section~\ref{sec:finiteK}; its last subsection
(Section~\ref{sec:recip}) proves Proposition~\ref{prop:recip}
(reciprocity and expansion in $K^{-2}$), independent of the rest.
\item Appendix~\ref{sec:pattern} proves the two statements about the harmonic component of the linear game made after
Proposition~\ref{prop:hflow} of the main text: the tie-pattern law (Theorem~\ref{thm:pattern-SM}) and the effect of
randomised tie-breaking (Proposition~\ref{prop:randtie-SM}).
\item Appendix~\ref{sec:cont} proves Theorem~\ref{thm:spectrum} (Hodge spectrum) and the identities
\eqref{eq:contquad}.
\item Appendix~\ref{sec:priced} proves the statement about priced priorities made after Corollary~\ref{cor:rigid} of
the main text (Proposition~\ref{prop:priced-SM}) and records the corresponding exact computation on the intersection.
\item Appendix~\ref{app:repro} lists the scripts behind every computer-assisted step, describes an end-to-end check
that certifies Theorem~\ref{thm:finiteK} for small $(K,N)$ without using any step of its proof, and says which
computations are \emph{not} part of any proof.
\end{itemize}
Proofs given in full in the main text (Lemma~\ref{lem:numop}, Proposition~\ref{prop:pairwise} and its corollary,
Propositions~\ref{prop:energies}, \ref{prop:hflow}, \ref{prop:fip}, \ref{prop:ne}
and~\ref{prop:learning}) are not repeated.


\begin{figure}[H]\centering
\includegraphics[width=\textwidth]{figs/figS_dependency.pdf}
\vspace{-8mm}
\caption{Logical structure of the supplementary material. Boxes are the fourteen steps of the proof of
Theorem~\ref{thm:finiteK} (Appendix~\ref{app:finiteK}); arrows point from a step to the steps that use it, and the
horizontal collector above Step~\ref{step:assembly} gathers everything the assembly needs: the higher orders
(Step~\ref{step:orders}), the kernel of $\mathrm{Sq}$ (Step~\ref{step:kerSq}), the three branches
(Steps~\ref{step:K5}--\ref{step:K3}) and the certificates (Step~\ref{step:certs}), which together cover every pair
$(K,N)$ with $K\ge3$; Step~\ref{step:B} feeds both the kernel statement and the image certificates. Dashed boxes are
the three computer-assisted steps; all computations are exact. Section~\ref{sec:recip} and
Appendices~\ref{sec:pattern}--\ref{sec:priced} are independent of the proof and of one another, except that
Appendix~\ref{sec:cont} uses the conservation law of Step~\ref{step:hoeff}.}\label{fig:dependency}
\end{figure}

\paragraph{What depends on what.} Figure~\ref{fig:dependency} shows the logical structure of this document. The four
appendices are independent of one another and depend on the main text only through Lemma~\ref{lem:numop} and the
definitions of Section~\ref{sec:setup}, except that Appendix~\ref{sec:cont} uses Lemma~\ref{lem:cons} of
Step~\ref{step:hoeff}; Section~\ref{sec:recip} is not used in the proof of Theorem~\ref{thm:finiteK}.



\paragraph{Conventions.} Notation is that of the main text. Throughout, $[N]=\{0,\dots,N-1\}$; functions on the
profile space $S$ carry the uniform probability measure and $\|g\|^2=\E[g^2]$; flows carry the counting inner
product $\langle x,y\rangle=\sum_ex(e)y(e)$; $A_i$ is the average over the $i$-th coordinate, $g_T$ the Hoeffding
component of $g$ on $T\subseteq[N]$, and $[u_i]_T$ that of the payoff $u_i$. The bond weights of Appendix~\ref{app:finiteK} are
$\mu_k=\frac{N-1-k}N$ and $\nu_k=\frac{k+1}N$, as in the main text; $\beta$ is reserved for the rationality parameter
and appears only in Appendix~\ref{sec:priced}. In Appendix~\ref{app:finiteK}
``Step~$k$'' refers to one of the fourteen steps of the proof of Theorem~\ref{thm:finiteK}, which are numbered in
reading order; parts of a single proof are labelled (1), (2), \dots\ and are local to that proof. Three kinds of
statement occur and are marked as such: results proved by hand; polynomial identities in $N$ established by computer
algebra, whose scripts are named at the point of use; and finitely many exact rational certificates. Nothing in any
proof depends on a floating-point computation.

\section{Proof of Theorem~\ref{thm:finiteK} (finite quantisation)}\label{app:finiteK}
Throughout this appendix the conflict graph is complete, $C=K_N$, the protocol is the index protocol, and
$u_i=f(\pos_i)$ for an arbitrary payoff-from-rank function $f$ with increments $F_j=f(j-1)-f(j)$; the factor $K^{N}$
between the expectation norm of functions and the counting norm of flows appears explicitly wherever one is
converted into the other. The proof is organised in fourteen steps, numbered in the order in which they are read; the five parts of the
architecture in Section~\ref{sec:finiteK} of the main text cite the steps they consist of.

\paragraph{Roadmap.} Table~\ref{tab:roadmap} lists the steps, what each proves, where its result is used, and how it
is verified. A reader interested only in the logical structure can read Steps~\ref{step:hoeff}--\ref{step:kerSq}
and~\ref{step:assembly} and take Table~\ref{tab:cov} on trust; a reader auditing the computer-assisted parts needs
Steps~\ref{step:K4}--\ref{step:certs} and Appendix~\ref{app:repro}.

\begin{table}[H]\centering\small
\caption{Roadmap of the proof of Theorem~\ref{thm:finiteK}. ``exact'' means rational or symbolic arithmetic.}
\label{tab:roadmap}
\begin{tabular}{@{}>{\raggedright\arraybackslash}p{0.06\linewidth}>{\raggedright\arraybackslash}p{0.40\linewidth}>{\raggedright\arraybackslash}p{0.22\linewidth}>{\raggedright\arraybackslash}p{0.26\linewidth}@{}}\toprule
step & proves & used in & verified by\\\midrule
\ref{step:hoeff} & Laplacian $\dv\delta=K\numop$, conservation, order decomposition $Q_K=K^{N+1}\sum_mQ^{(m)}_K$ (Lemmas~\ref{lem:lap}--\ref{lem:orderdec}) & every later step & by hand\\
\ref{step:B} & $Q_K\one=0$: the linear payoff is an exact null vector (Lemma~\ref{lem:B}) & kernel statement, Step~\ref{step:assembly} & by hand\\
\ref{step:orders} & $\|\sum_{i\in T}[u_i]_T\|^2\le2\sum_i\|[u_i]_T\|^2$, hence $Q^{(m)}_K\succeq0$ for $m\ge3$ (Proposition~\ref{prop:orders}, Lemma~\ref{lem:struct}) & reduces the theorem to $Q^{(1)}+Q^{(2)}\succeq0$ & by hand\\
\ref{step:bond} & bond vectors $\hat D_k(f)$; first- and second-order components in bond form (Propositions~\ref{prop:first}, \ref{prop:second}); $Q^{(1)}+Q^{(2)}=\fB_{N,K}(\hat D(f))$ (Proposition~\ref{thm:C}); injectivity on affine $f$ (Lemma~\ref{lem:transfer}) & Steps~\ref{step:SOS}--\ref{step:certs} work on $\fB$ alone & by hand\\
\ref{step:SOS} & Hahn--Poincar\'e and spread identities; the sum-of-squares identity $K^2\fB=\sum_kZ_k+\mathrm{Sq}-\mathrm{Neg}$ (Theorem~\ref{thm:SOS}) & Steps~\ref{step:kerSq}--\ref{step:K3} & by hand\\
\ref{step:kerSq} & $\mathrm{Sq}(D)=0$ iff $D\in\operatorname{span}(\one\otimes\one)$ (Lemma~\ref{lem:kerSq}) & kernel statement, Step~\ref{step:assembly} & by hand\\
\ref{step:Lstar} & sharp level inequality with constant $K-2$ (Lemma~\ref{lem:Lstar-SM}); the level pencil $\varrho(\mu)$ (Proposition~\ref{cor:rho}) & Steps~\ref{step:Sqlow}--\ref{step:K4} & by hand (Schur product)\\
\ref{step:Sqlow} & lower bound $\mathrm{Sq}\ge\mathrm{Sq}_{\rm low}$ in the bond vectors alone; step coordinates (Propositions~\ref{prop:Sqlow}, \ref{prop:hadamard}) & Step~\ref{step:perron} & by hand\\
\ref{step:perron} & Perron argument: $\fB\succeq0$ if condition (T) holds on every bond (Lemmas~\ref{lem:path}, \ref{lem:Zmatrix}, Proposition~\ref{prop:T}) & Steps~\ref{step:K5}--\ref{step:K4} & by hand ($M$-matrix criterion)\\
\ref{step:K5} & $K\ge5$: (T) from Lemma~\ref{lem:Lstar-SM} whenever $(N-2)(K-4)\ge4$ (Theorem~\ref{thm:K5}) & assembly & by hand\\
\ref{step:K4} & $K=4$: root isolation of the cubic for $\varrho(\mu)$, $\varrho\ge2\mu\nu+5(\mu\nu)^3$, hence (T) for $N\ge10$ (Lemma~\ref{lem:K4root}, Theorem~\ref{thm:K4}) & assembly & Sturm sequences; \texttt{audit\_\allowbreak K4.py} (exact)\\
\ref{step:K3} & $K=3$: block representation, shear, $C-\gamma I\succeq0$, Perron certificate for $N\ge17$ (Lemmas~\ref{lem:K3u}--\ref{lem:K3M}, Theorem~\ref{thm:K3}) & assembly & computer algebra, symbolic in $N$: \texttt{k3\_\allowbreak representation\_\allowbreak proof.py}, \texttt{s1\_\allowbreak closed.py}, \texttt{verify\_\allowbreak M\_\allowbreak symbolic.py} (exact)\\
\ref{step:certs} & the remaining pairs $(K,N)$ by exact $LDL^\top$ certificates on the bond space or on its image (Table~\ref{tab:cov}) & assembly & $25$ stored certificates; \texttt{verify\_\allowbreak certificates.py} (exact)\\
\ref{step:assembly} & assembly; $N=2$; the counterexample at $K=2$, $N=7$ & Theorem~\ref{thm:finiteK} & by hand; \texttt{k2\_\allowbreak witness.py} (exact)\\\bottomrule
\end{tabular}
\end{table}

\stepsection{hoeff}{Hoeffding decomposition, the number operator and conservation}\label{sec:hoeff}

This step fixes conventions and records, in the form used below, the facts behind Lemma~\ref{lem:numop} of the main
text. Throughout, $S=\{0,\dots,K-1\}^N$ carries the uniform probability measure and $\|g\|^2=\E[g^2]$ for functions
on~$S$; flows carry the counting inner product $\langle x,y\rangle=\sum_ex(e)y(e)$. For a function $g$ on~$S$ and a
coordinate~$i$, $A_i$ denotes averaging over~$s_i$. The Hoeffding
(ANOVA) decomposition is $g=\sum_{T\subseteq[N]}g_T$ with
$g_T=\prod_{j\in T}(I-A_j)\prod_{j\notin T}A_j\,g$; $g_T$ depends only on
$s_T$, has zero mean in each of its variables, and the $g_T$ are
mutually orthogonal. We write $g_m=\sum_{|T|=m}g_T$. The
\emph{number operator} $\numop=\sum_i(I-A_i)$ acts on $g_T$ as
multiplication by~$|T|$. On the complete graph we abbreviate
$\pos_i=\pos_{K_N}(i,s)$.

\begin{lemmaS}[Laplacian of the game graph]\label{lem:lap}
Let $\delta$ be the gradient and let $\delta^*$ be its adjoint. With the
divergence convention $(\dv x)(s)=\sum_{e\,\mathrm{into}\,s}x(e)-\sum_{e\,\mathrm{out\ of}\,s}x(e)$
one has $\langle\delta\phi,x\rangle=\langle\phi,\dv x\rangle$, i.e.\ $\delta^*=\dv$. Then
$\delta^*\delta=K\numop$; in particular $\delta^*\delta g_T=K|T|\,g_T$.
For the game flow $u$ of payoffs $(u_i)$,
\begin{equation}\label{eq:divS}
(\dv u)(s)=K\sum_i\big[u_i(s)-\bar u_i(s_{-i})\big],\qquad
\bar u_i:=A_iu_i,
\end{equation}
and the potential energy is
\begin{equation}\label{eq:specS}
\|\delta\phi^\star\|^2=K^{N}\sum_{m=1}^N\frac{\|(\dv u)_m\|^2}{mK}
=K^{N+1}\sum_{m=1}^N\frac{\|g_m\|^2}{m},\qquad g:=\sum_i(u_i-A_iu_i),
\end{equation}
which is the first identity of \eqref{eq:twoenergies} in the main text.
\end{lemmaS}
\begin{proof}
This is Lemma~\ref{lem:numop} of the main text, whose proof identifies $\dv\delta=K\numop$ and $\dv u=Kg$; the sum
over the $K^N$ profiles in $\langle\phi^\star,\dv\delta\phi^\star\rangle$ supplies the factor $K^N$ in
\eqref{eq:specS}, and diagonalising $\numop$ on the Hoeffding components gives the two forms.
\end{proof}

\begin{lemmaS}[conservation]\label{lem:cons}
For every conflict graph and every payoff-from-rank function~$f$,
$\sum_iu_i(s)$ is independent of~$s$ on the complete graph, and
$\sum_i\pos_C(i,s)=|E|$ on every graph. Consequently, on the complete
graph, $\sum_i[u_i]_T=0$ for every nonempty~$T$, hence
$g_T=\sum_{i\in T}[u_i]_T=-\sum_{i\notin T}[\bar u_i]_T$.
\end{lemmaS}
\begin{proof}
On $K_N$ the map $i\mapsto\pos_i$ is a permutation of
$\{0,\dots,N-1\}$ (the order by $(s_i,-i)$ is strict), so
$\sum_if(\pos_i)=\sum_rf(r)$. On a general graph each conflict edge
contributes exactly one unit to the position of whichever endpoint is
served second. A constant has no nonconstant Hoeffding components, which
gives $\sum_i[u_i]_T=0$; finally $[u_i]_T$ with $i\notin T$ equals
$[\bar u_i]_T$ because $[u_i]_T$ contains the factor $A_i$.
\end{proof}

\begin{lemmaS}[order decomposition]\label{lem:orderdec}
For every $f$,
\begin{equation}\label{eq:P2}
\|u\|^2=K^{N+1}\sum_i\sum_{T\ni i}\|[u_i]_T\|^2,\qquad
\|Pu\|^2=K^{N+1}\sum_{T\ne\emptyset}\frac1{|T|}\Big\|\sum_{i\in T}[u_i]_T\Big\|^2 .
\end{equation}
Consequently $F^\top Q_KF=K^{N+1}\sum_{m\ge1}Q^{(m)}_K(f)$ with
\begin{equation}\label{eq:Qm-SM}
Q^{(m)}_K(f)=\sum_{|T|=m}\Big[\frac{N-1}N\sum_{i\in T}\|[u_i]_T\|^2-\frac1m\Big\|\sum_{i\in T}[u_i]_T\Big\|^2\Big],
\end{equation}
which is \eqref{eq:Qm} of the main text.
\end{lemmaS}
\begin{proof}
Since $I-A_i$ annihilates the Hoeffding components on sets not containing $i$ and fixes the others,
$u_i-A_iu_i=\sum_{T\ni i}[u_i]_T$, an orthogonal sum; this gives the first identity by Lemma~\ref{lem:numop}. Summing
over $i$ and collecting by index set, $g=\sum_i(u_i-A_iu_i)$ has components $g_T=\sum_{i\in T}[u_i]_T$, and the second
identity is again Lemma~\ref{lem:numop}. The last statement is the definition
$Q_K=\frac{N-1}NM_{\mathrm{tot}}-M_\pot$ with $F^\top M_{\mathrm{tot}}F=\|u\|^2$ and $F^\top M_\pot F=\|Pu\|^2$
(flow norms).
\end{proof}

\stepsection{B}{proof of Lemma~\ref{lem:B} (exact eigenvector)}\label{sec:lemA}

With the order decomposition in place, the first thing to establish is that the linear payoff is an exact null
vector of $Q_K$ at every finite $K$. The result is used twice: for the kernel statement of
Theorem~\ref{thm:finiteK} (Step~\ref{step:assembly}), and inside the certificates of Step~\ref{step:certs}, which need to know that the bond
form annihilates the linear payoff.

\begin{mainlem}[\ref{lem:B} of the main text]
For every $N\ge2$ and $K\ge2$, $Q_K\one=0$, i.e.\
$M_\pot\one=\frac{N-1}NM_{\mathrm{tot}}\one$.
\end{mainlem}

Players are indexed $0,\dots,N-1$, so player $i$ has exactly $i$
opponents of smaller index. Write $u^{\rm lin}$ for the flow of the linear
game and $u^f$ for that of $\mathcal G_f(K_N,K)$.

\emph{(1) Reduction.}
By definition of the Gram matrices, $Q_K\one=0$ is equivalent to
$\langle Pu^{\rm lin}-\frac{N-1}Nu^{\rm lin},\,u^f\rangle=0$ for all $f$.
By Proposition~\ref{prop:energies} with $d_i\equiv N-1$, $Pu^{\rm lin}=\delta\phi$ with
$\phi=\frac{N-1}K\sum_is_i$, which on the edges of player~$i$ is the
flow of the payoff $(N-1)\phi_1(s_i)$, $\phi_1(a):=\frac{a-\bar s}K$,
$\bar s=\frac{K-1}2$. Writing $-\pos_i=\sum_{j\ne i}\psi_{ij}(s_i,s_j)$ with
$\psi_{ij}(a,b)=-\one[b>a]$ ($j>i$) or $-\one[b\ge a]$ ($j<i$), the
Hoeffding decomposition of each kernel is
$\psi_{ij}=\bar\psi_{ij}+\phi_1(a)-\phi_1(b)+\Gamma_{ij}(a,b)$ (both kernels have
the same first-order parts $\phi_1(a)$ and $-\phi_1(b)$; this is checked
directly: $\E_b\psi_{ij}(a,b)$ equals $-\frac{K-1-a}K$ or
$-\frac{K-a}K$, both equal to $\frac{a-\bar s}K$ up to a constant).
Hence $u^{\rm lin}$ is the flow of $(N-1)\phi_1(s_i)+\Gamma_i$ with
$\Gamma_i:=\sum_{j\ne i}\Gamma_{ij}(s_i,s_j)$, and the harmonic part
$h=u^{\rm lin}-\delta\phi$ is the flow of $\Gamma_i$. For two payoff
families $(w_i)$, $(v_i)$ the inner product of their flows is
\begin{equation}\label{eq:flowip}
\langle\text{flow}(w),\text{flow}(v)\rangle
=\sum_i\sum_{s_{-i}}\sum_{a<b}\big(w_i(b)-w_i(a)\big)\big(v_i(b)-v_i(a)\big)
=K^{N+1}\sum_i\E\big[\Cov(w_i,v_i\mid s_{-i})\big],
\end{equation}
since $\sum_{a<b}(x_b-x_a)(y_b-y_a)=K^2\Cov(x,y)$ for the uniform law on
$\{0,\dots,K-1\}$. Because $\Gamma_i$ and $\phi_1(s_i)$ are centred in
$s_i$ for every $s_{-i}$, the conditional covariances reduce to plain
expectations, and the claim becomes
\begin{equation}\label{eq:B1}
\sum_i\E[\Gamma_i\,v_i]=\sum_i\E[\phi_1(s_i)\,v_i]\qquad\text{for all }f,
\end{equation}
where $v_i=f(\pos_i)$.

\emph{(2) Using conservation.}
Let $\Xi_i=\sum_{j\ne i}(-\phi_1(s_j))$ be the second-variable first-order
part, so that $-\pos_i=-\E\pos_i+\allowbreak(N-1)\phi_1(s_i)+\Xi_i+\Gamma_i$. By Lemma~\ref{lem:cons},
$\sum_i\E[\Xi_iv_i]=\allowbreak-\sum_j\E\big[\phi_1(s_j)\sum_{i\ne j}v_i\big]
=-\sum_j\E\big[\phi_1(s_j)(\mathrm{const}-v_j)\big]=\sum_j\E[\phi_1(s_j)v_j]$.
Therefore
$\sum_i\E[\Gamma_iv_i]=\allowbreak\sum_i\E[(\E\pos_i-\pos_i)v_i]-N\sum_i\E[\phi_1(s_i)v_i]$,
and \eqref{eq:B1} is equivalent to
\begin{equation}\label{eq:B2}
\sum_i\E[\pos_i]\,\E[f(\pos_i)]-\sum_{r}r f(r)
=\frac{N+1}K\sum_i\Cov\big(s_i,f(\pos_i)\big),
\end{equation}
where we used $\sum_i\E[\pos_if(\pos_i)]=\sum_rrf(r)$ (Lemma~\ref{lem:cons}).

\emph{(3) Generating functions.}
Both sides of \eqref{eq:B2} are linear in $f$, so it suffices to take
$f(r)=x^r$. Put $y=x-1$. Given $s_i$, write $\hat a=K-1-s_i$; opponent $j<i$
is served before $i$ with probability $\frac{\hat a+1}K$ and opponent $j>i$
with probability $\frac{\hat a}K$, independently across~$j$. Let
$\mathsf B_{\hat a}=1+\frac{\hat a}Ky$ and $\mathsf A_{\hat a}=1+\frac{\hat a+1}Ky=\mathsf B_{\hat a+1}$. Then
\[
\Pi_i(x):=\E[x^{\pos_i}]=\frac1K\sum_{\hat a=0}^{K-1}\mathsf A_{\hat a}^{\,i}\mathsf B_{\hat a}^{\,N-1-i},\qquad
\mu_i:=\E[\pos_i]=\frac{(N-1)\frac{K-1}2+i}K .
\]
With $\sum_{i=0}^{N-1}\mathsf A^i\mathsf B^{N-1-i}=\frac{\mathsf A^N-\mathsf B^N}{\mathsf A-\mathsf B}$, $\mathsf A_{\hat a}-\mathsf B_{\hat a}=\frac yK$,
telescoping ($\mathsf A_{\hat a}=\mathsf B_{\hat a+1}$, $\mathsf B_0=1$, $\mathsf B_K=1+y$), $\mathsf S:=\sum_{\hat a=0}^K\mathsf B_{\hat a}^N$
and $G(x):=\sum_{r=0}^{N-1}x^r=\frac{(1+y)^N-1}y$:
\begin{align*}
\sum_i\Pi_i&=\frac1y\sum_{\hat a=0}^{K-1}(\mathsf A_{\hat a}^N-\mathsf B_{\hat a}^N)=G,\\
\sum_ii\,\Pi_i&=\frac1y\sum_{\hat a=0}^{K-1}(N\mathsf A_{\hat a}^N+\mathsf B_{\hat a}^N)-\frac{K\big((1+y)^{N+1}-1\big)}{y^2}\\
 &=\frac{(N+1)\mathsf S-N-(1+y)^N}{y}-\frac{K\big((1+y)^{N+1}-1\big)}{y^2},\\
Z(x)&:=\sum_i\E[s_ix^{\pos_i}]=\frac1y\sum_{\hat a=0}^{K-1}(K-1-\hat a)(\mathsf A_{\hat a}^N-\mathsf B_{\hat a}^N)\\
 &=\frac{\mathsf S-K-(1+y)^N}{y}.
\end{align*}
(The second line uses $\sum_ii\,\mathsf A^i\mathsf B^{N-1-i}=\mathsf A\partial_{\mathsf A}\frac{\mathsf A^N-\mathsf B^N}{\mathsf A-\mathsf B}$;
the third is a summation by parts: with $\mathsf A_{\hat a}=\mathsf B_{\hat a+1}$,
$\sum_{\hat a=0}^{K-1}(K-1-\hat a)(\mathsf B_{\hat a+1}^N-\mathsf B_{\hat a}^N)=\sum_{\hat a=1}^{K-1}\mathsf B_{\hat a}^N-(K-1)\mathsf B_0^N
=\mathsf S-\mathsf B_0^N-\mathsf B_K^N-(K-1)$, and $\mathsf B_0^N=1$, $\mathsf B_K^N=(1+y)^N$.) The generating-function form of
\eqref{eq:B2} is $\sum_i\mu_i\Pi_i-xG'=\frac{N+1}K\big(Z-\frac{K-1}2G\big)$.
Substituting, $\mathsf S$ and $K$ cancel and the difference of the two sides equals
\begin{align*}
NG+\frac{N+1}y-\frac{(1+y)^{N+1}-1}{y^2}-xG'
&=\frac{Ny(1+y)^N+y-(1+y)^{N+1}+1}{y^2}\\
&\quad-\frac{Ny(1+y)^N-(1+y)^{N+1}+1+y}{y^2}=0 .
\end{align*}
This proves \eqref{eq:B2}, hence Lemma~\ref{lem:B}. \qed

\begin{remarkS}
The quantisation $K$ disappears in part (3): the identity only uses that,
conditionally on $s_i$, the opponents are served before $i$ independently,
and that positions form a permutation. 
\end{remarkS}

\stepsection{orders}{proof of Proposition~\ref{prop:orders} (higher orders)}\label{sec:orders}
The order decomposition of Lemma~\ref{lem:orderdec} splits $Q_K$ into a sum over Hoeffding orders $m$. This step
disposes of every order $m\ge3$ at once, by an argument that uses nothing about $f$; what remains afterwards is the
two-body form $Q^{(1)}_K+Q^{(2)}_K$, which occupies Steps~\ref{step:bond}--\ref{step:certs}.

\begin{mainprop}[\ref{prop:orders} of the main text]
For all $N\ge3$, $K\ge2$ and $m\ge3$, $Q^{(m)}_K\succeq0$, where
\[
Q^{(m)}_K(f)=\frac{N-1}N\sum_{|T|=m}\sum_{i\in T}\|[u_i]_T\|^2-\frac1m\sum_{|T|=m}\Big\|\sum_{i\in T}[u_i]_T\Big\|^2 .
\]
More precisely, for every $T$ with $|T|=m$,
$\big\|\sum_{i\in T}[u_i]_T\big\|^2\le2\sum_{i\in T}\|[u_i]_T\|^2$, and the
constant~$2$ cannot be improved at $K=2$.
\end{mainprop}

\noindent Here $Q^{(m)}_K$ is viewed as a quadratic form in the increments~$F$ of~$f$; since
$F^\top Q_KF=K^{N+1}\sum_mQ^{(m)}_K(f)$ by Lemma~\ref{lem:orderdec}, positive-semidefiniteness statements about the
$Q^{(m)}_K$ transfer to $Q_K$ unchanged.

\begin{lemmaS}[structure of the components]\label{lem:struct}
Let $T=\{i_1<\dots<i_m\}$ and $i\in T$. Put $t^{(i)}_j(a)=a$ for $j>i$ and
$a-1$ for $j<i$, $\theta(x;t)=\one[x>t]$, $p(t)=\frac{K-1-t}K$ (with
$p(-1)=1$). Then
\[
[u_i]_T=(I-A_i)F_i,\qquad
F_i(s_T)=\Psi^{(i)}(s_T)\,D^{(i)}(s_i),\qquad
\Psi^{(i)}=\prod_{j\in T\setminus i}\big(\theta(s_j;t^{(i)}_j(s_i))-p(t^{(i)}_j(s_i))\big),
\]
with $D^{(i)}(a)=\E\big[\Delta^{m-1}f(B^{(a)}_{\notin T})\big]$, where
$B^{(a)}_{\notin T}$ is the number of players outside $T$ served before~$i$
when $s_i=a$.
\end{lemmaS}
\begin{proof}
We have $\pos_i=\sum_{j\in T\setminus i}\theta(s_j;t^{(i)}_j(s_i))+B_{\notin T}$.
Averaging over the coordinates outside $T$ gives
$\E f\big(\sum_{j\in T\setminus i}\theta_j+B\big)$. For $j\in T\setminus i$
and any function $\zeta$, $\zeta(\theta_j)=\zeta(0)+\theta_j\Delta\zeta(0)$ because
$\theta_j\in\{0,1\}$, so $(I-A_j)\zeta(\theta_j)=(\theta_j-p_j)\Delta\zeta(0)$;
applying this successively to all $j\in T\setminus i$ produces the product
$\Psi^{(i)}$ and the $(m-1)$-fold difference, and $(I-A_i)$ is the last
factor.
\end{proof}

\begin{proof}[Proof of Proposition~\ref{prop:orders}]
Fix $T$, write $X_i=[u_i]_T=(I-A_i)F_i$. Three facts.

\emph{(i) Cross terms.} For $i\ne k$ in $T$, $F_k$ is centred in $s_i$ (it
contains the factor $\theta(s_i;\cdot)-p$), so $A_iF_k=0$ and, $A_i$ being
an orthogonal projection, $\langle A_iF_i,F_k\rangle=\langle A_iF_i,A_iF_k\rangle=0$;
similarly the other cross projections vanish, whence
$\langle X_i,X_k\rangle=\langle F_i,F_k\rangle$.

\emph{(ii) The cross kernel is entrywise nonpositive.} For $i<k$,
conditioning on $s_i=a$, $s_k=b$ and averaging over the remaining
coordinates,
\begin{gather*}
\langle F_i,F_k\rangle=\frac1{K^2}\sum_{a,b}D^{(i)}(a)D^{(k)}(b)\,\Omega_{ik}(a,b),\\
\Omega_{ik}(a,b)=-\big(\one[b>a]-p(a)\big)\big(\one[b>a]-q(b)\big)\prod_{j\ne i,k}\dk\big(t^{(i)}_j(a),t^{(k)}_j(b)\big),
\end{gather*}
with $q(b)=b/K$ and $\dk(t,t')=p(\max(t,t'))-p(t)p(t')\ge0$. Indeed the
factor of $\Psi^{(i)}$ involving $s_k$ is $\one[b>a]-p(a)$ (as $k>i$), and
the factor of $\Psi^{(k)}$ involving $s_i$ is
$\one[a\ge b]-p(b-1)=-(\one[b>a]-q(b))$ (as $i<k$, $p(b-1)=1-q(b)$): the two
indicators are complementary, so the product is $-(1-p)(1-q)\le0$ if $b>a$
and $-pq\le0$ if $b\le a$. The remaining factors are covariances of two
increasing indicators of the same variable, hence nonnegative.

\emph{(iii) Diagonal terms.} $\|X_i\|^2=\|F_i\|^2-\|A_iF_i\|^2$, where
$\|F_i\|^2$ depends on $D^{(i)}$ only through $D^{(i)}(a)^2$, and
$\|A_iF_i\|^2=\frac1{K^2}\sum_{a,a'}D^{(i)}(a)D^{(i)}(a')\Omega^{\rm d}_i(a,a')$ with
$\Omega^{\rm d}_i(a,a')=\prod_{j\ne i}\dk(t^{(i)}_j(a),t^{(i)}_j(a'))\ge0$.

Let $\tilde D^{(i)}=|D^{(i)}|$ and $\tilde F_i,\tilde X_i$ the corresponding
vectors. By (i)--(ii),
\begin{align*}
\sum_{i\ne k}\langle X_i,X_k\rangle
&\le\frac1{K^2}\sum_{i\ne k}\sum_{a,b}|D^{(i)}(a)|\,|D^{(k)}(b)|\,|\Omega_{ik}(a,b)|
=-\sum_{i\ne k}\langle\tilde F_i,\tilde F_k\rangle\\
&=\sum_i\|\tilde X_i\|^2-\Big\|\sum_i\tilde X_i\Big\|^2\le\sum_i\|\tilde X_i\|^2 .
\end{align*}
By (iii), $\|\tilde X_i\|^2\le\|X_i\|^2$. Therefore
\[
\Big\|\sum_iX_i\Big\|^2=\sum_i\|X_i\|^2+\sum_{i\ne k}\langle X_i,X_k\rangle
\le2\sum_i\|X_i\|^2 .
\]
Summing over $T$,
\[
\sum_{|T|=m}\|g_T\|^2\le2\sum_{|T|=m}\sum_{i\in T}\|[u_i]_T\|^2,\qquad\text{so}\qquad
Q^{(m)}_K\ge\Big(\frac{N-1}N-\frac2m\Big)\sum_{|T|=m}\sum_{i\in T}\|[u_i]_T\|^2\ge0
\]
as soon as $m\ge\frac{2N}{N-1}$, i.e.\ $m\ge3$ for $N\ge3$. For $K=2$ the
interior members of $T$ have $X_i=0$ (their $\Psi^{(i)}$ vanishes at both
levels) and the two extreme members are parallel; for $f$ chosen so that they have equal norm and the same
orientation the inequality is an equality, so the constant~$2$ cannot be improved.
\end{proof}

%=====================================================================================================
\stepsection{bond}{bond vectors and the two-body reduction (first part of Proposition~\ref{prop:bond})}\label{sec:bond}
The two-body form $Q^{(1)}_K+Q^{(2)}_K$ is a quadratic form in the $N-1$ increments of $f$. This step rewrites it as a
quadratic form $\fB_{N,K}$ in $N-1$ \emph{bond vectors} $\hat D_k(f)\in\R^K$, one for each pair of adjacent positions,
whose entries are averaged first differences of $f$. The point of the change of variables is that $\fB_{N,K}$ is
defined on all of $(\R^K)^{N-1}$, not only on the image $\{\hat D(f)\}$, and positivity on the larger space is what
Steps~\ref{step:SOS}--\ref{step:K3} prove; Lemma~\ref{lem:transfer} at the end of this step brings the kernel back to $f$.

\paragraph{Notation for the rest of the appendix.} Levels are $a\in\{0,\dots,K-1\}$ and carry the uniform probability
measure; $\Var$ and $\Cov$ of functions of the level refer to it. \emph{Bonds} are indexed by $k\in\{0,\dots,N-2\}$. For
$D\in\R^K$ we write
\[
(J_1D)(a)=\sum_{x\le a}D(x),\qquad (J_0D)(a)=\sum_{x<a}D(x),
\]
for the inclusive and exclusive cumulative sums, written without the operators in the main text; given bond vectors
$D_0,\dots,D_{N-2}\in\R^K$ we put $G_k=J_1D_k$, $H_k=J_0D_k$, so that $G_k-H_k=D_k$, and define the \emph{vertex
functions}
\begin{equation}\label{eq:Omega}
\Omega_j:=\sum_{k<j}H_k+\sum_{k\ge j}G_k,\qquad j=0,\dots,N-1 ,
\end{equation}
which satisfy $\Omega_k-\Omega_{k+1}=D_k$. Further $\mu_k=\frac{N-1-k}N$, $\nu_k=\frac{k+1}N$ (so that $\nu_k+\mu_l=1-\frac{l-k}N$ for $k\le l$; in particular $\mu_k+\nu_k=1$), and
\begin{equation}\label{eq:Hahn}
\calD(g)=\sum_{y=1}^{K-1}\frac{y(K-y)}K\big(g(y)-g(y-1)\big)^2,\qquad P(g):=\calD(g)-\Var(g),
\end{equation}
is the Hahn Dirichlet form. For a payoff-from-rank function $f$, with $\Delta f(r)=f(r+1)-f(r)$, the \emph{bond vectors
of $f$} are
\begin{equation}\label{eq:Dhat}
\hat D_k(a)=\E\Big[\Delta f\Big(\Bin\big(k,\tfrac{K-a}K\big)+\Bin\big(N-2-k,\tfrac{K-1-a}K\big)\Big)\Big],
\end{equation}
the two binomials being independent. The \emph{bond form} is the quadratic form on $(\R^K)^{N-1}$
\begin{equation}\label{eq:formula1}
K^2\fB_{N,K}(D):=\underbrace{\frac{N-2}{2}\sum_k\big[\mu_kP(H_k)+\nu_kP(G_k)\big]}_{\mathrm I}
+\underbrace{\sum_{k\le l}\Cov(H_k,G_l)}_{\mathrm{II}}
-\underbrace{\frac1N\sum_{j=0}^{N-1}\Var(\Omega_j)}_{\mathrm{III}} .
\end{equation}

\begin{lemmaS}[what an opponent sees]\label{lem:groups}
Conditionally on $s_i=a$, the events ``$j$ is served before $i$'', $j\ne i$, are independent; their probability is
$\frac{K-a}K$ for $j<i$ (the event $s_j\ge a$) and $\frac{K-1-a}K$ for $j>i$ (the event $s_j>a$). Moreover, for any
random variable $R$ with values in $\{0,\dots,N-2\}$, independent of the Bernoulli variables below, and any
$p\in[0,1-\frac1K]$,
\begin{equation}\label{eq:oneflip}
\E f\big(R+\mathrm{Bern}(p+\tfrac1K)\big)-\E f\big(R+\mathrm{Bern}(p)\big)=\tfrac1K\,\E\,\Delta f(R).
\end{equation}
\end{lemmaS}
\begin{proof}
The first statement is the definition \eqref{eq:pos} of the index protocol together with the independence of the
levels. For the second, $\E f(R+\mathrm{Bern}(p))=\E f(R)+p\,\E\Delta f(R)$ is affine in $p$.
\end{proof}

\begin{propS}[first order]\label{prop:first}
Let $\varphi_j(a):=\E[u_j\mid s_j=a]$ and let $\Omega_j$ be built from the bond vectors \eqref{eq:Dhat} of $f$. Then
$\varphi_j=-\frac1K\Omega_j+\mathrm{const}$, and
\begin{equation}\label{eq:Q1}
Q^{(1)}_K(f)=-\frac1N\sum_{j=0}^{N-1}\Var(\varphi_j)=-\frac1{NK^2}\sum_{j=0}^{N-1}\Var(\Omega_j).
\end{equation}
\end{propS}
\begin{proof}
By Lemma~\ref{lem:groups}, given $s_j=a$ the position of $j$ is a sum of $j$ independent Bernoulli variables of
parameter $\frac{K-a}K$ (the opponents of smaller index) and $N-1-j$ of parameter $\frac{K-1-a}K$. Passing from level
$a$ to level $a-1$ raises every parameter by $\frac1K$; we do this one opponent at a time, in two stages, applying
\eqref{eq:oneflip} at each flip with $R$ the contribution of the other $N-2$ opponents.
\emph{Stage (i):} raise the $N-1-j$ opponents of larger index from $\frac{K-1-a}K$ to $\frac{K-a}K$. When $m$ of the
other $N-2$ opponents are at $\frac{K-a}K$ and $N-2-m$ at $\frac{K-1-a}K$, the increment is $\frac1K\hat D_m(a)$ by
\eqref{eq:Dhat}; here $m$ runs from $j$ to $N-2$.
\emph{Stage (ii):} all opponents are now at $\frac{K-a}K=\frac{K-1-(a-1)}K$; raise the $j$ opponents of smaller index
to $\frac{K-(a-1)}K$. When $m$ of the others have been raised the increment is $\frac1K\hat D_m(a-1)$, $m=0,\dots,j-1$.
Hence
\[
\varphi_j(a-1)-\varphi_j(a)=\frac1K\Big[\sum_{m\ge j}\hat D_m(a)+\sum_{m<j}\hat D_m(a-1)\Big]
=\frac1K\big[\Omega_j(a)-\Omega_j(a-1)\big],
\]
because $G_m(a)-G_m(a-1)=\hat D_m(a)$ and $H_m(a)-H_m(a-1)=\hat D_m(a-1)$. This gives the first claim. For
\eqref{eq:Q1}, $[u_j]_{\{j\}}=\varphi_j-\E\varphi_j$ and, in \eqref{eq:Qm-SM} with $m=1$,
$\frac{N-1}N\|[u_j]_{\{j\}}\|^2-\|[u_j]_{\{j\}}\|^2=-\frac1N\Var(\varphi_j)$.
\end{proof}

\begin{propS}[second order]\label{prop:second}
Let $i<j$, $X_i:=[u_i]_{\{i,j\}}$ and $X_j:=[u_j]_{\{i,j\}}$, and let $H_k,G_k$ be built from the bond vectors of $f$.
Then
\begin{equation}\label{eq:second}
\|X_i\|^2=\frac{P(H_i)}{K^2},\qquad \|X_j\|^2=\frac{P(G_{j-1})}{K^2},\qquad
\langle X_i,X_j\rangle=-\frac{\Cov(H_i,G_{j-1})}{K^2}.
\end{equation}
\end{propS}
\begin{proof}
Write $a=s_i$, $b=s_j$, let $A_a,A_b$ be the averaging operators in these coordinates and $C_a=I-A_a$, $C_b=I-A_b$; they
are commuting orthogonal projections. Put $p(t)=\frac{K-1-t}K$, so that $\E_b\one[b>t]=p(t)$ for $-1\le t\le K-1$.

\emph{The component $X_i$.} Given $a$ and $b$, $\pos_i=\one[b>a]+R$, where $R$ is the contribution of the other $N-2$
opponents: $i$ of smaller index and $N-2-i$ of larger index, so by Lemma~\ref{lem:groups}
$\E[f(R+1)-f(R)\mid a]=\hat D_i(a)$ and
$\E[u_i\mid a,b]=\chi(a)+\one[b>a]\hat D_i(a)$ with $\chi(a)=\E[f(R)\mid a]$. Now $X_i=C_aC_b\E[u_i\mid a,b]$; $C_b$
annihilates $\chi(a)$, and $C_b[\one[b>a]\hat D_i(a)]=(\one[b>a]-p(a))\hat D_i(a)=:F(a,b)$. Thus $X_i=C_aF$ with $F$
centred in $b$, and $\|X_i\|^2=\|F\|^2-\|A_aF\|^2$. First,
\[
\|F\|^2=\frac1K\sum_ap(a)(1-p(a))\hat D_i(a)^2=\frac1{K^2}\sum_{a=0}^{K-2}\frac{(a+1)(K-1-a)}K\hat D_i(a)^2=\frac{\calD(H_i)}{K^2},
\]
since $H_i(y)-H_i(y-1)=\hat D_i(y-1)$. Second, $\sum_a\one[b>a]\hat D_i(a)=H_i(b)$ and
$\sum_ap(a)\hat D_i(a)=\E_bH_i(b)$, so $(A_aF)(b)=\frac1K(H_i(b)-\E H_i)$ and $\|A_aF\|^2=\Var(H_i)/K^2$. This proves
the first identity.

\emph{The component $X_j$.} Symmetrically, given $a,b$ one has $\pos_j=\one[a\ge b]+R'$, where the other opponents of $j$
are $j-1$ of smaller index and $N-1-j$ of larger index, so that the coefficient is $\hat D_{j-1}(b)$, and
$X_j=C_b\tilde F$ with $\tilde F(a,b)=(\one[a\ge b]-p(b-1))\hat D_{j-1}(b)$, centred in $a$. Here
$p(b-1)(1-p(b-1))=\frac{b(K-b)}{K^2}$ and $G_{j-1}(y)-G_{j-1}(y-1)=\hat D_{j-1}(y)$ give
$\|\tilde F\|^2=\calD(G_{j-1})/K^2$, while $\sum_b\one[a\ge b]\hat D_{j-1}(b)=G_{j-1}(a)$ gives
$\|A_b\tilde F\|^2=\Var(G_{j-1})/K^2$.

\emph{The cross term.} Since $C_a$ is self-adjoint, $C_aC_b=C_bC_a$, $C_a\tilde F=\tilde F$ and $C_bF=F$,
\[
\langle C_aF,C_b\tilde F\rangle=\langle F,C_bC_a\tilde F\rangle=\langle F,C_b\tilde F\rangle=\langle C_bF,\tilde F\rangle
=\langle F,\tilde F\rangle .
\]
The two indicators are complementary, $\one[a\ge b]=1-\one[b>a]$ and $p(b-1)=1-\E_U\one[U\ge b]$, whence
\[
\big(\one[b>a]-p(a)\big)\big(\one[a\ge b]-p(b-1)\big)=-\big(\one[b>a]-p(a)\big)\big(\one[b>a]-\tfrac bK\big).
\]
Checking the cases $b>a$ and $b\le a$ separately, the right-hand side equals
$-\dk(a,b-1)$, where $\dk(t,t'):=\Cov_U(\one[U>t],\one[U>t'])=p(\max(t,t'))-p(t)p(t')\ge0$ for $U$ uniform on the levels.
Therefore
\[
\langle X_i,X_j\rangle=-\frac1{K^2}\sum_{a,b}\hat D_i(a)\hat D_{j-1}(b)\,\Cov_U\big(\one[U>a],\one[U\ge b]\big)
=-\frac1{K^2}\Cov\big(H_i(U),G_{j-1}(U)\big).\qedhere
\]
\end{proof}

\begin{propS}[two-body reduction; Proposition~\ref{prop:bond} of the main text]\label{thm:C}
For every $N\ge2$, $K\ge2$ and every payoff-from-rank function $f$,
$Q^{(1)}_K(f)+Q^{(2)}_K(f)=\fB_{N,K}\big(\hat D(f)\big)$.
\end{propS}
\begin{proof}
For $m=2$, \eqref{eq:Qm-SM} reads
$Q^{(2)}_K=\sum_{i<j}\big[\frac{N-2}{2N}(\|X_i\|^2+\|X_j\|^2)-\langle X_i,X_j\rangle\big]$, since
$\frac{N-1}N-\frac12=\frac{N-2}{2N}$. By \eqref{eq:second}, bond $k$ occurs through $P(H_k)$ in the $N-1-k$ pairs $(k,j)$,
$j>k$, and through $P(G_k)$ in the $k+1$ pairs $(i,k+1)$, $i\le k$; this gives $K^{-2}\,\mathrm I$. The map
$(i,j)\mapsto(k,l)=(i,j-1)$ is a bijection from $\{i<j\}$ onto $\{k\le l\}$, so the cross terms give $K^{-2}\,\mathrm{II}$.
Finally $Q^{(1)}_K=-K^{-2}\,\mathrm{III}$ by \eqref{eq:Q1}.
\end{proof}

\begin{lemmaS}[kernel transfer]\label{lem:transfer}
$\hat D(f)\in\operatorname{span}(\one\otimes\one)$, i.e.\ $\hat D_k(a)=c$ for all $k$ and $a$, if and only if $f$ is
affine.
\end{lemmaS}
\begin{proof}
If $\Delta f\equiv c$ then $\hat D_k\equiv c$ by \eqref{eq:Dhat}. Conversely, at the top level $a=K-1$ the second binomial
in \eqref{eq:Dhat} is degenerate at $0$, so $\hat D_k(K-1)=\E\,\Delta f(\Bin(k,\frac1K))$, $k=0,\dots,N-2$. This is a
triangular linear system in $\Delta f(0),\dots,\Delta f(N-2)$ with diagonal entries $K^{-k}>0$; its unique solution with
right-hand side $c\,\one$ is $\Delta f\equiv c$.
\end{proof}

Proposition~\ref{thm:C} uses only exchangeability within the two index groups, the one-flip identity and the orthogonality of
the Hoeffding projections. It holds for every $K\ge2$, including $K=2$, where Theorem~\ref{thm:finiteK} fails: the
hypothesis $K\ge3$ enters only through Lemma~\ref{lem:Lstar-SM} below.

%=====================================================================================================
\stepsection{SOS}{the sum-of-squares identity \texorpdfstring{\eqref{eq:SOS}}{of the main text}}\label{sec:SOS}
The bond form \eqref{eq:formula1} has one negative term, $\mathrm{III}$, of the same order as the two positive ones. This
step rearranges the three terms into a sum of manifestly nonnegative pieces plus a single negative term of a
different shape, $-\sum_kc_k\Var(D_k)$, which involves the bond vectors only through their variances; every later step
is a way of paying for that term. Two elementary identities are needed first.

\begin{lemmaS}[Hahn--Poincar\'e]\label{lem:hahn}
For every function $g$ of the level, $\calD(g)=\sum_{m=1}^{K-1}m(m+1)\Var_m(g)$, where $\Var_m(g)$ is the squared norm of
the component of $g$ along the discrete Chebyshev polynomial of degree $m$ on $\{0,\dots,K-1\}$. In particular
$\calD(g)\ge2\Var(g)$, with equality iff $g$ is affine.
\end{lemmaS}
\begin{proof}
Summation by parts gives $\calD(g)=\E[g\cdot Lg]$ with
$(Lg)(y)=-\big[(y+1)(K-1-y)(g(y+1)-g(y))-y(K-y)(g(y)-g(y-1))\big]$, the second-order difference operator of the Hahn
polynomials with parameters $(0,0)$, whose eigenfunctions are the discrete Chebyshev polynomials with eigenvalues
$m(m+1)$ \cite[Sec.~9.5]{koekoek2010}. The components of degree $m\ge2$ have eigenvalue at least $6>2$.
\end{proof}

\begin{lemmaS}[spread identity]\label{lem:spread}
For functions $z_0,\dots,z_{n-1}$ of the level,
$n\sum_k\Var(z_k)-\Var\big(\sum_kz_k\big)=\sum_{k<l}\Var(z_k-z_l)$.
\end{lemmaS}
\begin{proof}
Both sides equal $(n-1)\sum_k\Var(z_k)-2\sum_{k<l}\Cov(z_k,z_l)$.
\end{proof}

\begin{thmS}[sum-of-squares identity]\label{thm:SOS}
For all bond vectors $D_0,\dots,D_{N-2}\in\R^K$,
\begin{equation}\label{eq:SOS-SM}
K^2\fB_{N,K}(D)=\sum_kZ_k+\mathrm{Sq}(D)-\sum_kc_k\Var(D_k),\qquad c_k:=2N\mu_k\nu_k-\tfrac12 ,
\end{equation}
where $Z_k:=\frac{N-2}2\big[\mu_k(\calD-2\Var)(H_k)+\nu_k(\calD-2\Var)(G_k)\big]\ge0$ and
\begin{equation}\label{eq:Sq-SM}
\mathrm{Sq}(D):=\frac1{2N}\sum_{k<l}\Big[(N{-}1{-}l)\Var(H_k-H_l+D_l)+(k{+}1)\Var(G_k-G_l+D_k)+(l{-}k)\Var(H_k-G_l)\Big]\ge0 .
\end{equation}
\end{thmS}
\begin{proof}
\emph{1) Vertex variables.} For $j\in\{0,\dots,N-1\}$ and a bond $k$ put $Z_{jk}:=H_k$ if $k<j$ and $Z_{jk}:=G_k$ if
$k\ge j$, so that $\Omega_j=\sum_kZ_{jk}$, and let $\E_j$ denote the average over $j$. For fixed $k$, $Z_{jk}=H_k$ for the
$N-1-k$ values $j>k$ and $Z_{jk}=G_k$ for the $k+1$ values $j\le k$. Hence, in \eqref{eq:formula1},
\[
\mathrm I=\tfrac{N-2}2\,\E_j\sum_kP(Z_{jk}),\qquad \mathrm{III}=\E_j\Var\Big(\sum_kZ_{jk}\Big),\qquad
\sum_kZ_k=\tfrac{N-2}2\,\E_j\sum_k(\calD-2\Var)(Z_{jk}).
\]
\emph{2) Spreading.} With $n=N-1$ bonds, Lemma~\ref{lem:spread} gives, for each $j$,
\[
\tfrac{N-2}2\sum_kP(Z_{jk})=\tfrac{N-2}2\sum_k(\calD-2\Var)(Z_{jk})+\tfrac12\sum_{k<l}\Var(Z_{jk}-Z_{jl})
-\tfrac12\sum_k\Var(Z_{jk})+\tfrac12\Var(\Omega_j);
\]
indeed both sides equal $\frac{N-2}2\sum_k\calD(Z_{jk})-\frac{N-2}2\sum_k\Var(Z_{jk})$. Averaging over $j$ and inserting
into \eqref{eq:formula1},
\begin{equation}\label{eq:SOSmid}
K^2\fB=\sum_kZ_k+\tfrac12\E_j\sum_{k<l}\Var(Z_{jk}-Z_{jl})+\Xi,\qquad
\Xi:=\mathrm{II}-\tfrac12\E_j\Big[\Var(\Omega_j)+\sum_k\Var(Z_{jk})\Big].
\end{equation}
\emph{3) The pair term.} For $k<l$ the pair $(Z_{jk},Z_{jl})$ equals $(G_k,G_l)$ for the $k+1$ values $j\le k$,
$(H_k,G_l)$ for the $l-k$ values $k<j\le l$, and $(H_k,H_l)$ for the $N-1-l$ values $j>l$. Therefore
\begin{equation}\label{eq:pairterm}
\tfrac12\E_j\sum_{k<l}\Var(Z_{jk}-Z_{jl})=\frac1{2N}\sum_{k<l}\Big[(k{+}1)\Var(G_k-G_l)+(l{-}k)\Var(H_k-G_l)+(N{-}1{-}l)\Var(H_k-H_l)\Big].
\end{equation}
\emph{4) The residual.} Since $\frac12[\Var(\Omega_j)+\sum_k\Var(Z_{jk})]=\sum_k\Var(Z_{jk})+\sum_{k<l}\Cov(Z_{jk},Z_{jl})$,
the same count gives
\[
\Xi=\sum_{k<l}\Big[\big(1-\tfrac{l-k}N\big)\Cov(H_k,G_l)-\nu_k\Cov(G_k,G_l)-\mu_l\Cov(H_k,H_l)\Big]
+\sum_k\Big[\Cov(H_k,G_k)-\mu_k\Var(H_k)-\nu_k\Var(G_k)\Big].
\]
As $1-\frac{l-k}N=\nu_k+\mu_l$ and $G=H+D$, the first bracket is $\mu_l\Cov(H_k,D_l)-\nu_k\Cov(G_l,D_k)$; as
$\mu_k+\nu_k=1$, the second is $\mu_k\Cov(H_k,D_k)-\nu_k\Cov(G_k,D_k)=(\mu_k-\nu_k)\Cov(H_k,D_k)-\nu_k\Var(D_k)$.
Thus
\begin{equation}\label{eq:Xi}
\Xi=\sum_{k<l}\big[\mu_l\Cov(H_k,D_l)-\nu_k\Cov(G_l,D_k)\big]+\sum_k\big[(\mu_k-\nu_k)\Cov(H_k,D_k)-\nu_k\Var(D_k)\big].
\end{equation}
\emph{5) Absorption.} Expanding the shifted variances and using
$2\Cov(H,D)=\Var(G)-\Var(H)-\Var(D)$,
\begin{align}
\tfrac12\Var(H_k-H_l)+\Cov(H_k,D_l)&=\tfrac12\Var(H_k-H_l+D_l)+\tfrac12\big[\Var G_l-\Var H_l\big]-\Var(D_l),\label{eq:abs1}\\
\tfrac12\Var(G_k-G_l)-\Cov(G_l,D_k)&=\tfrac12\Var(G_k-G_l+D_k)-\tfrac12\big[\Var G_k-\Var H_k\big]-\Var(D_k).\label{eq:abs2}
\end{align}
The weights match: the $(H,H)$ pair carries $\frac{N-1-l}{2N}=\frac{\mu_l}2$ in \eqref{eq:pairterm} and $\mu_l$ in
\eqref{eq:Xi}, the $(G,G)$ pair $\frac{\nu_k}2$ and $\nu_k$. Applying \eqref{eq:abs1}--\eqref{eq:abs2} converts
\eqref{eq:pairterm} plus the off-diagonal part of \eqref{eq:Xi} into $\mathrm{Sq}(D)$ plus multiples of
$\frac12(\Var G_k-\Var H_k)$ and of $\Var(D_k)$, which we now collect together with the diagonal part of \eqref{eq:Xi},
written as $(\mu_k-\nu_k)\cdot\frac12(\Var G_k-\Var H_k)-\frac{\mu_k-\nu_k}2\Var(D_k)-\nu_k\Var(D_k)$.

\emph{Coefficient of $\frac12(\Var G_k-\Var H_k)$.} Bond $k$ is the second index of $k$ pairs, each contributing
$+\mu_k$ by \eqref{eq:abs1}, and the first index of $N-2-k$ pairs, each contributing $-\nu_k$ by \eqref{eq:abs2}; the
diagonal contributes $\mu_k-\nu_k$. The total is
$\frac1N\big[k(N-1-k)-(k+1)(N-2-k)+(N-2-2k)\big]=0$.

\emph{Coefficient of $\Var(D_k)$.} The same three sources give $-k\mu_k$, $-(N-2-k)\nu_k$ and
$-\frac{\mu_k-\nu_k}2-\nu_k=-\frac12$, and
$\frac{k(N-1-k)+(k+1)(N-2-k)}N+\frac12=\frac{2(N-1-k)(k+1)}N-\frac12=c_k$.

\emph{6) Signs.} $Z_k\ge0$ by Lemma~\ref{lem:hahn}, and $\mathrm{Sq}\ge0$ because its weights are nonnegative.
\end{proof}

%=====================================================================================================
\stepsection{kerSq}{the kernel of \texorpdfstring{$\mathrm{Sq}$}{Sq}}\label{sec:kerSq}
The term $\mathrm{Sq}$ of Theorem~\ref{thm:SOS} is what pins down the kernel of $\fB_{N,K}$: once positivity is known,
$\fB(D)=0$ forces $\mathrm{Sq}(D)=0$, and the following lemma turns that into $D\in\operatorname{span}(\one\otimes\one)$.
It is used in the kernel part of Proposition~\ref{prop:T} and in the assembly (Step~\ref{step:assembly}).

\begin{lemmaS}[kernel of $\mathrm{Sq}$]\label{lem:kerSq}
Let $N\ge3$, $K\ge2$. If $\mathrm{Sq}(D)=0$ then $D\in\operatorname{span}(\one\otimes\one)$: there is $c\in\R$ with
$D_k=c\,\one$ for every bond $k$.
\end{lemmaS}
\begin{proof}
On the range $0\le k<l\le N-2$ the three weights in \eqref{eq:Sq-SM} are at least $1$. Hence $\mathrm{Sq}(D)=0$ forces,
for every pair $k<l$, each of $H_k-G_l$, $H_k-H_l+D_l$ and $G_k-G_l+D_k$ to be constant in the level. Using
$H(a+1)-H(a)=D(a)$ and $G(a+1)-G(a)=D(a+1)$ and taking first differences at $a=0,\dots,K-2$:
\[
D_k(a)=D_l(a+1),\qquad D_k(a)-2D_l(a)+D_l(a+1)=0,\qquad 2D_k(a+1)-D_l(a+1)-D_k(a)=0 .
\]
Substituting the first relation into the second gives $D_l(a+1)=D_l(a)$, so $D_l$ is constant whenever $l$ occurs as a
second index; substituting it into the third gives $D_k(a+1)=D_k(a)$, so $D_k$ is constant whenever $k$ occurs as a first
index. Since $N\ge3$ there are at least two bonds, and every bond is a first index ($k\le N-3$) or a second index
($l\ge1$); so $D_k=c_k\one$ for all $k$, and the first relation gives $c_k=c_l$.
\end{proof}
All three groups of squares are needed: the first alone does not constrain $D_0(K-1)$ nor $D_{N-2}(0)$; the second removes
the latter freedom and the third the former.

%=====================================================================================================
\stepsection{Lstar}{the sharp level inequality (Lemma~\ref{lem:Lstar})}\label{sec:Lstar}
The terms $Z_k$ of Theorem~\ref{thm:SOS} are nonnegative by Lemma~\ref{lem:hahn}, but that alone does not pay for
$-c_k\Var(D_k)$. This step shows that $Z_k$ dominates $\Var(D_k)$ with an explicit constant, and that the constant
carries the factor $K-2$: this is the one place where the hypothesis $K\ge3$ enters.

\begin{lemmaS}[sharp level inequality]\label{lem:Lstar-SM}
For every $K\ge3$, $\mu\in[0,1]$, $\nu=1-\mu$ and $D\in\R^K$,
\begin{equation}\label{eq:Lstar-SM}
\mu(\calD-2\Var)(J_0D)+\nu(\calD-2\Var)(J_1D)\ \ge\ (K-2)\,\mu\nu\,\Var(D),
\end{equation}
and the constant $K-2$ cannot be improved. Moreover, in the step coordinates $c_m=D(m)-D(m-1)$, $m=1,\dots,K-1$, the
difference of the two sides of \eqref{eq:Lstar-SM} equals $\frac2{K^2}\,c^\top\big[(Kg)\circ\Phi_\mu\big]c$, where
$g(m,m')=\min(m,m')(K-\max(m,m'))/K$ is the Green's function of the Dirichlet Laplacian of the path
$\{1,\dots,K-1\}$ and $\Phi_\mu=\widetilde M_\mu-\frac{K\mu\nu}2\one\one^\top$ is positive semidefinite, with
\begin{equation}\label{eq:Mtilde}
\widetilde M_\mu(m,m')=\tilde a_{\min(m,m')}\tilde b_{\max(m,m')},\qquad
\tilde a_m=\frac{m-1+2\mu}2,\quad\tilde b_m=\frac{K-m-1+2\nu}2 .
\end{equation}
\end{lemmaS}
\begin{proof}
\emph{1) Pair representation.} Let $\Phi=J_1D$ and, for $1\le y\le y'\le K-1$,
$\gamma(y,y'):=\frac yK\big(1-\frac{y'}K\big)$. Since
$\Var(\Phi)=\frac1{K^2}\sum_{a<b}\big(\sum_{a<y\le b}D(y)\big)^2$ under the uniform law on the levels, the coefficient
of $D(y)D(y')$, $y\le y'$, in $\Var(\Phi)$ is $\frac1{K^2}\#\{(a,b):a<y,\ b\ge y'\}=\gamma(y,y')$ (counted twice if
$y<y'$). Writing
$D(y)D(y')=\frac12(D(y)^2+D(y')^2)-\frac12(D(y)-D(y'))^2$,
\[
\Var(\Phi)=\sum_{y\ge1}D(y)^2\Big[\gamma(y,y)+\sum_{y'\ne y}\gamma(\min,\max)\Big]-\sum_{1\le y<y'}\gamma(y,y')\big(D(y)-D(y')\big)^2 .
\]
A direct summation gives $\sum_{y'\ne y}\gamma(\min,\max)=\frac{K-2}2\gamma(y,y)$, while $\calD(\Phi)=K\sum_y\gamma(y,y)D(y)^2$.
Hence the diagonal terms cancel in $\calD-2\Var$ and
\[
(\calD-2\Var)(J_1D)=\frac2{K^2}\sum_{1\le y<y'\le K-1}y\,(K-y')\,\big(D(y)-D(y')\big)^2 .
\]
The same computation for $J_0D$, which is $J_1D$ shifted by one level, gives
$(\calD-2\Var)(J_0D)=\frac2{K^2}\sum_{0\le y<y'\le K-2}(y+1)(K-1-y')(D(y)-D(y'))^2$.

\emph{2) The pencil.} For $0\le y<y'\le K-1$ (both weights vanish outside the ranges above),
\[
\mu(y+1)(K-1-y')+\nu\,y(K-y')=(y+\mu)(K-\mu-y')-\mu\nu ,
\]
an identity in $(y,y',\mu)$. Since $\Var(D)=\frac1{K^2}\sum_{y<y'}(D(y)-D(y'))^2$, \eqref{eq:Lstar-SM} is equivalent to
\begin{equation}\label{eq:pencil}
\sum_{0\le y<y'\le K-1}\Big[(y+\mu)(K-\mu-y')-\tfrac K2\mu\nu\Big]\big(D(y)-D(y')\big)^2\ \ge0 .
\end{equation}
\emph{3) Step coordinates.} With $D(y')-D(y)=\sum_{y<m\le y'}c_m$, the left-hand side of \eqref{eq:pencil} is
$c^\top\mathcal Kc$ with, for $m\le m'$,
\[
\mathcal K(m,m')=\sum_{y<m,\ y'\ge m'}\Big[(y+\mu)(K-\mu-y')-\tfrac K2\mu\nu\Big]
=m(K-m')\Big[\tilde a_m\tilde b_{m'}-\tfrac K2\mu\nu\Big],
\]
because $\sum_{y<m}(y+\mu)=m\tilde a_m$ and $\sum_{y'\ge m'}(K-\mu-y')=(K-m')\tilde b_{m'}$. Thus
$\mathcal K=(Kg)\circ\Phi_\mu$.

\emph{4) $\Phi_\mu\succeq0$.} Let $0<\mu<1$. The sequences $\tilde a$ and $\tilde b$ are positive, $\tilde a$
increasing and $\tilde b$ decreasing, with constant Wronskian
$\tilde a_{m+1}\tilde b_m-\tilde a_m\tilde b_{m+1}=\frac12(\tilde a_m+\tilde b_m)=\frac K4$. The inverse of such a one-pair
(Green) matrix is tridiagonal \cite[Ch.~II, pp.~78--79 and 103--104]{gantmacher2002}: $\widetilde T:=\widetilde M_\mu^{-1}$ has off-diagonal
entries $-\frac4K$, interior diagonal entries $\frac8K$, and corner entries $\frac4K(1+\frac1{2\mu})$ and
$\frac4K(1+\frac1{2\nu})$. That is, $\widetilde T=\frac4K\big[L_{\rm path}+\operatorname{diag}(\frac1{2\mu},0,\dots,0,\frac1{2\nu})\big]\succ0$,
with $L_{\rm path}$ the Neumann Laplacian of the path; in particular
$\one^\top\widetilde T\one=\frac4K\big(\frac1{2\mu}+\frac1{2\nu}\big)=\frac2{K\mu\nu}$. For a positive definite
$M$, $c\,\one\one^\top\succeq0$ iff $c\,\one^\top M^{-1}\one\le1$; with $c=\frac K2\mu\nu$ equality holds, so
$\Phi_\mu\succeq0$, with one-dimensional kernel. The cases $\mu\in\{0,1\}$ follow by continuity.

\emph{5) Schur product.} $g\succeq0$ and $\Phi_\mu\succeq0$, so $\mathcal K=(Kg)\circ\Phi_\mu\succeq0$ by the Schur
product theorem. Sharpness of the constant $K-2$: take $D=e_0$ and let $\mu\to0$.
\end{proof}

\begin{propS}[the level pencil]\label{cor:rho}
For $0<\mu<1$ let $\varrho(\mu)$ be the smallest generalised eigenvalue of the pencil
$\big((Kg)\circ\widetilde M_\mu,\,Kg\big)$, and let $c^\star(\mu)$ be the largest constant that can replace
$(K-2)\mu\nu$ in \eqref{eq:Lstar-SM}. Then $\varrho(\mu)=\mu\nu+\tfrac12c^\star(\mu)$, which is the definition
used in the main text, and $\varrho(\mu)\ge\frac K2\mu\nu$.
\end{propS}
\begin{proof}
By part 3) of the preceding proof and $\Var(D)=K^{-2}c^\top(Kg)c$, the left-hand side of \eqref{eq:Lstar-SM} equals
$\frac2{K^2}c^\top[(Kg)\circ\widetilde M_\mu]c-2\mu\nu\Var(D)$, so $\mathrm{LHS}\ge\lambda\Var(D)$ holds for all
$D$ iff $(Kg)\circ\widetilde M_\mu\succeq(\mu\nu+\frac\lambda2)Kg$; hence $c^\star=2\varrho-2\mu\nu$. Finally
$(Kg)\circ\widetilde M_\mu-\frac K2\mu\nu\,(Kg)=(Kg)\circ\Phi_\mu\succeq0$, and $Kg\succ0$.
\end{proof}

%=====================================================================================================
\stepsection{Sqlow}{a lower bound in the bond vectors alone, and step coordinates}\label{sec:Sqlow}
The identity \eqref{eq:SOS-SM} has a single negative term, $-\sum_kc_k\Var(D_k)$, which involves the bond vectors only
through their covariances. We bound the two positive terms from below by quantities of the same kind.

\begin{lemmaS}[minimising out a common part]\label{lem:minout}
Let $w_1,\dots,w_r>0$ with $\sum_iw_i=W$, and let $Y_1,\dots,Y_r$ be functions of the level. For every function $X$ of
the level,
$\sum_iw_i\Var(X+Y_i)\ \ge\ \sum_iw_i\Var(Y_i)-\frac1W\Var\big(\sum_iw_iY_i\big)$.
\end{lemmaS}
\begin{proof}
$\sum_iw_i\Var(X+Y_i)=W\Var(X)+2\Cov(X,\bar Y)+\sum_iw_i\Var(Y_i)$ with $\bar Y=\sum_iw_iY_i$, and
$W\Var(X)+2\Cov(X,\bar Y)=W\Var(X+\bar Y/W)-\Var(\bar Y)/W\ge-\Var(\bar Y)/W$.
\end{proof}

\begin{propS}[the bond matrix]\label{prop:Sqlow}
Let $g_b(k,l):=\frac{(\min(k,l)+1)(N-1-\max(k,l))}N$, $0\le k,l\le N-2$, and
\begin{equation}\label{eq:Pbond}
\mathsf P:=2(N-1)\operatorname{diag}(\mu_k\nu_k)-\tfrac2N\,g_b .
\end{equation}
Then $\mathrm{Sq}(D)\ \ge\ \mathrm{Sq}_{\rm low}(D):=\sum_{k,l}\mathsf P_{kl}\Cov(D_k,D_l)$ for all bond vectors.
\end{propS}
\begin{proof}
Fix $k<l$ and put $X=H_k-H_l$, $a=N-1-l$, $b=k+1$, $c=l-k$, so that $a+b+c=N$. Since $G=H+D$, the three functions in
\eqref{eq:Sq-SM} are $X+D_l$, $X+2D_k-D_l$ and $X-D_l$, with weights $a,b,c$. By Lemma~\ref{lem:minout}, and because
$aD_l+b(2D_k-D_l)-cD_l=2bD_k+(2a-N)D_l$, the pair $(k,l)$ contributes to $2N\,\mathrm{Sq}$ at least
\[
(a+c)\Var(D_l)+b\Var(2D_k-D_l)-\tfrac1N\Var\big(2bD_k+(2a-N)D_l\big)
=\tfrac{4a(N-a)}N\Var(D_l)+\tfrac{4b(N-b)}N\Var(D_k)-\tfrac{8ab}N\Cov(D_k,D_l),
\]
where we used $N-\frac{(2a-N)^2}N=\frac{4a(N-a)}N$ and $-4b-\frac{4b(2a-N)}N=-\frac{8ab}N$. Now $a=N\mu_l$,
$N-a=N\nu_l$, $b=N\nu_k$, $N-b=N\mu_k$; dividing by $2N$, the pair contributes at least
$2\mu_l\nu_l\Var(D_l)+2\mu_k\nu_k\Var(D_k)-4\nu_k\mu_l\Cov(D_k,D_l)$. Each bond belongs to $N-2$ pairs,
which gives the diagonal $2(N-2)\mu_k\nu_k=2(N-1)\mu_k\nu_k-\frac2Ng_b(k,k)$, and for $k<l$ the symmetric
off-diagonal entry is $-2\nu_k\mu_l=-\frac2Ng_b(k,l)$.
\end{proof}

\begin{propS}[step coordinates]\label{prop:hadamard}
Let $c_k\in\R^{K-1}$, $c_k(m)=D_k(m)-D_k(m-1)$, and let $g$, $\widetilde M_\mu$ be as in Lemma~\ref{lem:Lstar-SM}. Then
$\Cov(D_k,D_l)=K^{-2}c_k^\top(Kg)c_l$, and
\begin{equation}\label{eq:F}
K^2\Big[\sum_kZ_k+\mathrm{Sq}_{\rm low}-\sum_kc_k\Var(D_k)\Big]
=(N-2)\sum_kc_k^\top\big[(Kg)\circ\widetilde M_{\mu_k}\big]c_k+\sum_{k,l}\Lambda_{kl}\,c_k^\top(Kg)\,c_l,
\end{equation}
with $\Lambda:=\mathsf P-\operatorname{diag}\big((N-2)\mu_k\nu_k+c_k\big)$, where in the last expression $c_k=2N\mu_k\nu_k-\frac12$
is the scalar of \eqref{eq:SOS-SM}.
\end{propS}
\begin{proof}
$\Cov(D,D')=\frac1{K^2}\sum_{y<y'}(D(y')-D(y))(D'(y')-D'(y))$, and the coefficient of $c(m)c'(m')$, $m\le m'$, in this sum
is $\#\{y<m\}\cdot\#\{y'\ge m'\}=m(K-m')=Kg(m,m')$. By Lemma~\ref{lem:Lstar-SM},
$\mu(\calD-2\Var)(J_0D)+\nu(\calD-2\Var)(J_1D)=\frac2{K^2}c^\top[(Kg)\circ\Phi_\mu]c+(K-2)\mu\nu\Var(D)$, and
$(Kg)\circ\Phi_\mu=(Kg)\circ\widetilde M_\mu-\frac{K\mu\nu}2Kg$; hence
\[
K^2Z_k=(N-2)\,c_k^\top\big[(Kg)\circ\widetilde M_{\mu_k}\big]c_k-(N-2)\mu_k\nu_k\,c_k^\top(Kg)c_k .
\]
Add $K^2\mathrm{Sq}_{\rm low}=\sum_{k,l}\mathsf P_{kl}c_k^\top(Kg)c_l$ and $-K^2c_k\Var(D_k)=-c_k\,c_k^\top(Kg)c_k$.
\end{proof}

%=====================================================================================================
\stepsection{perron}{a Perron argument in the space of bonds}\label{sec:perron}
Proposition~\ref{prop:hadamard} has reduced positivity of $\fB_{N,K}$ to positivity of a block matrix on the space
of bonds whose blocks are Hadamard products with the fixed positive definite matrix $Kg$. This step shows that the
whole matrix is positive as soon as a scalar condition, (T) below, holds on every bond; the condition is then checked
branch by branch in Steps~\ref{step:K5}--\ref{step:K4}. Let $L$ be the Dirichlet Laplacian of the path with vertices $0,\dots,N-2$ (diagonal $2$, off-diagonal $-1$), and recall
$\varrho(\mu)$ from Proposition~\ref{cor:rho}.

\begin{lemmaS}\label{lem:path}
$g_b=L^{-1}$, and the positive vector $v_k=(k+1)(N-1-k)=N^2\mu_k\nu_k$ satisfies $Lv=2\cdot\one$.
\end{lemmaS}
\begin{proof}
$g_b$ is the Green's function of the Dirichlet problem on the path; $v$ is quadratic in $k$ with second difference $-2$
and vanishes at $k=-1$ and $k=N-1$.
\end{proof}

\begin{lemmaS}[symmetric $Z$-matrices]\label{lem:Zmatrix}
Let $M$ be a real symmetric matrix with $M_{ij}\le0$ for $i\ne j$, and let $v$ have positive entries. For every $x$,
\begin{equation}\label{eq:Zid}
x^\top Mx=\sum_i\frac{(Mv)_i}{v_i}x_i^2+\frac12\sum_{i\ne j}(-M_{ij})\,v_iv_j\Big(\frac{x_i}{v_i}-\frac{x_j}{v_j}\Big)^2 .
\end{equation}
Hence $Mv\ge0$ implies $M\succeq0$; if moreover $M$ is irreducible and $Mv\ne0$, then $M\succ0$.
\end{lemmaS}
\begin{proof}
Expand the square and use $\sum_jM_{ij}v_j=(Mv)_i$. If $x^\top Mx=0$ with $M$ irreducible, the second sum forces
$x=t\,v$, and then the first gives $t^2v^\top Mv=0$, so $t=0$ when $Mv\ne0$.
\end{proof}

\begin{propS}[condition (T)]\label{prop:T}
Let $N\ge3$, $K\ge3$, and put $\theta_k:=(N-2)\varrho(\mu_k)-N\mu_k\nu_k+\frac12$. If, for every bond $k$,
\begin{equation}\label{eq:T-SM}
(N-2)\,\varrho(\mu_k)-2N\mu_k\nu_k+\tfrac12\ \ge\ 0,\tag{T}
\end{equation}
then $\fB_{N,K}\succeq0$. If in addition \eqref{eq:T-SM} is strict for at least one bond, then
$\ker\fB_{N,K}=\operatorname{span}(\one\otimes\one)$.
\end{propS}
\begin{proof}
By Theorem~\ref{thm:SOS} and Propositions~\ref{prop:Sqlow} and~\ref{prop:hadamard},
$K^2\fB=(\mathrm{Sq}-\mathrm{Sq}_{\rm low})+K^{-2}\mathcal F(c)$ with $\mathcal F$ the right-hand side of \eqref{eq:F}, and
$\mathrm{Sq}-\mathrm{Sq}_{\rm low}\ge0$.
By definition of $\varrho$, $(Kg)\circ\widetilde M_{\mu_k}\succeq\varrho(\mu_k)\,Kg$, so
$\mathcal F(c)\ge\sum_{k,l}\mathsf A_{kl}\,c_k^\top(Kg)c_l$ with
$\mathsf A:=\operatorname{diag}\big((N-2)\varrho(\mu_k)\big)+\Lambda$. Inserting \eqref{eq:Pbond},
\[
\mathsf A=\operatorname{diag}(\theta_k)-\tfrac2N\,g_b=\operatorname{diag}(\theta_k)-\tfrac2N\,L^{-1}.
\]
Since $Kg\succ0$, the form $\sum_{k,l}\mathsf A_{kl}c_k^\top(Kg)c_l=c^\top(\mathsf A\otimes Kg)c$ is nonnegative iff
$\mathsf A\succeq0$. Condition \eqref{eq:T-SM} says $\theta_k\ge N\mu_k\nu_k>0$. For $\Theta=\operatorname{diag}(\theta_k)\succ0$,
$\Theta\succeq\frac2NL^{-1}$ is equivalent to $\frac N2L\succeq\Theta^{-1}$, i.e.\ to $\mathsf M:=NL-2\Theta^{-1}\succeq0$.
$\mathsf M$ is a symmetric $Z$-matrix and, by Lemma~\ref{lem:path},
$(\mathsf Mv)_k=2N-\frac{2v_k}{\theta_k}=\frac{2N}{\theta_k}\big(\theta_k-N\mu_k\nu_k\big)\ge0$,
so $\mathsf M\succeq0$ by Lemma~\ref{lem:Zmatrix}, and $\fB\succeq0$.

For the kernel, let $\fB(D)=0$. If \eqref{eq:T-SM} is strict for some bond, then $\mathsf Mv\ne0$; $L$ is irreducible, so
$\mathsf M\succ0$, hence $\mathsf A\succ0$ and $\mathsf A\otimes Kg\succ0$. As both $\mathrm{Sq}-\mathrm{Sq}_{\rm low}$ and
$\mathcal F$ are nonnegative, $\mathcal F(c)=0$, so $c=0$: every bond vector is constant in the level, $D_k=t_k\one$. Then
$H_k(a)=t_ka$, $G_k(a)=t_k(a+1)$, $\mathrm{Sq}_{\rm low}(D)=0$ and
$\mathrm{Sq}(D)=\frac1{2N}\sum_{k<l}N(t_k-t_l)^2\Var(a)$, which vanishes only if all $t_k$ coincide. Conversely
$\fB(\one\otimes\one)=0$ by Proposition~\ref{thm:C} and Lemma~\ref{lem:B} applied to the linear payoff, for which all
$Q^{(m)}_K$, $m\ge3$, vanish.
\end{proof}

%=====================================================================================================
\stepsection{K5}{the branch \texorpdfstring{$K\ge5$}{K>=5}}\label{sec:K5}
For $K\ge5$ the lower bound $\varrho(\mu)\ge\frac K2\mu\nu$ of Proposition~\ref{cor:rho} verifies (T) for all but
finitely many $N$.
\begin{thmS}\label{thm:K5}
Let $K\ge5$ and $N\ge3$ with $(N-2)(K-4)\ge4$. Then $\fB_{N,K}\succeq0$ with kernel $\operatorname{span}(\one\otimes\one)$.
Explicitly this covers $N\ge6$ for $K=5$, $N\ge4$ for $K=6,7$, and $N\ge3$ for $K\ge8$.
\end{thmS}
\begin{proof}
Write $x=\mu_k\nu_k\in(0,\frac14]$. By Proposition~\ref{cor:rho}, $\varrho(\mu_k)\ge\frac K2x$, so the left-hand side of
\eqref{eq:T-SM} is at least $x\,s+\frac12$ with $s:=\frac{(N-2)K}2-2N$. If $s\ge0$ this is positive. If $s<0$ it is at
least $\frac s4+\frac12=\frac18\big[(N-2)(K-4)-4\big]\ge0$, with strict inequality unless $x=\frac14$. Since
$\mu_k\nu_k=\frac14$ for at most one bond and there are $N-1\ge2$ bonds, \eqref{eq:T-SM} is strict for some bond, and
Proposition~\ref{prop:T} applies.
\end{proof}
\emph{Where the argument stops.} At $K=4$ the bracket is $(N-2)\cdot0-4<0$ for every $N$: the bound $\varrho\ge\frac K2\mu\nu$ is never sufficient, and the
true value of $\varrho$ is needed. At $K=3$ even that fails (Step~\ref{step:K3}). The three-branch case distinction is therefore forced by the problem, not by the method.

%=====================================================================================================
\stepsection{K4}{the branch \texorpdfstring{$K=4$}{K=4} (computer-assisted root isolation)}\label{sec:K4}
For $K=4$ the pencil of Proposition~\ref{cor:rho} is $3\times3$ and
$\det\big((Kg)\circ\widetilde M_\mu-\varrho\,Kg\big)=-4\,\mathcal P(\varrho;\mu)$ with
\begin{align*}
\mathcal P(\varrho;\mu)={}&4\varrho^3-10\varrho^2+6\varrho+12\mu^4\varrho-24\mu^3\varrho+12\mu^2\varrho^2-13\mu^2\varrho-12\mu\varrho^2+25\mu\varrho\\
&+4\mu^6-12\mu^5-3\mu^4+26\mu^3-3\mu^2-12\mu .
\end{align*}

\begin{lemmaS}\label{lem:K4root}
For every $\mu\in(0,1)$, $\varrho(\mu)$ is the unique root of $\mathcal P(\cdot;\mu)$ in $(0,\frac7{10})$, and
\begin{equation}\label{eq:rho0}
\varrho(\mu)\ >\ \varrho_0(\mu):=2\mu\nu+5(\mu\nu)^3 .
\end{equation}
\end{lemmaS}
\begin{proof}
All three roots are positive, because both matrices of the pencil are positive definite. The following facts about
polynomials in $\mu$ with rational coefficients are established by exact root counting (Sturm sequences; script
\texttt{audit\_K4.py}): (i) $\mathcal P(0;\mu)=\mu(1-\mu)q_0(\mu)$ with $\deg q_0=4$ and $q_0<0$ on $[0,1]$;
(ii) $\mathcal P(\frac7{10};\mu)$, of degree $6$, has no root in $[0,1]$ and equals $\frac{51}{500}>0$ at $\mu=\frac12$;
(iii) $\mathcal P(\varrho_0(\mu);\mu)=[\mu(1-\mu)]^2q_1(\mu)$ with $\deg q_1=14$ and $q_1<0$ on $[0,1]$. Moreover
the three roots sum to $\frac52+3\mu(1-\mu)\ge\frac52>3\cdot\frac7{10}$, so they are not all below $\frac7{10}$. With the
positive leading coefficient, (i) and (ii) give exactly one root in $(0,\frac7{10})$ and two above; it is $\varrho(\mu)$.
Since $\varrho_0\le\frac{37}{64}<\frac7{10}$ and $\mathcal P<0$ on $(0,\varrho(\mu))$, (iii) gives $\varrho_0(\mu)<\varrho(\mu)$.
\end{proof}
The bound \eqref{eq:rho0} is nearly tight ($\min_\mu[\varrho-\varrho_0]\approx8\times10^{-7}$), which is why $K=4$ needs it.

\begin{thmS}\label{thm:K4}
For $K=4$ and $N\ge10$, $\fB_{N,4}\succeq0$ with kernel $\operatorname{span}(\one\otimes\one)$.
\end{thmS}
\begin{proof}
With $x=\mu_k\nu_k$ and \eqref{eq:rho0}, the left-hand side of \eqref{eq:T-SM} exceeds
$(N-2)(2x+5x^3)-2Nx+\frac12=5(N-2)x^3-4x+\frac12=:f_N(x)$; the linear terms collapse to $-4x$ independently of $N$. On
$x>0$, $f_N$ is minimised at $x_*^2=\frac4{15(N-2)}$, where $f_N(x_*)=\frac12-\frac83x_*$. This is nonnegative iff
$x_*\le\frac3{16}$, i.e.\ iff $N-2\ge\frac{1024}{135}=7.58\ldots$, i.e.\ iff $N\ge10$. So \eqref{eq:T-SM} holds strictly
for every bond, and Proposition~\ref{prop:T} applies.
\end{proof}
The threshold is sharp for this route: for $3\le N\le9$ condition \eqref{eq:T-SM} with the exact $\varrho$ fails at some
bond. Those cases, and the finitely many cases left open by Theorem~\ref{thm:K5}, are settled by exact certificates in
Step~\ref{step:certs}.

%=====================================================================================================
\stepsection{K3}{the branch \texorpdfstring{$K=3$}{K=3} (computer-assisted)}\label{sec:K3}
For $K=3$ the lower bound $\mathrm{Sq}\ge\mathrm{Sq}_{\rm low}$ is too lossy: the form \eqref{eq:F} is indefinite, with
smallest eigenvalue of order $-N/10$. The part $X=H_k-H_l$ discarded in Proposition~\ref{prop:Sqlow} must be kept, and we
work with the bond form itself. The argument has a fixed architecture, proved by hand, and a small number of closed forms
for matrix entries which are polynomial identities in $(N,i,j)$ established by computer algebra.

\paragraph{Representation.} The level space is $\R^3$ with basis $\one$, $t_1=(-1,0,1)$, $t_2=(1,-2,1)$. Write
$D_k=u_k\one+s_kt_1+q_kt_2$ and order the coordinates as $(u,s,q)\in(\R^{N-1})^3$, bonds being indexed by
$i=k+1\in\{1,\dots,N-1\}$. Let $T$ be the matrix of the quadratic form $K^2\fB_{N,3}$ in these coordinates, with blocks
$T_{uu},T_{ur},T_{rr}$, $r=(s,q)$.

\begin{lemmaS}[block representation]\label{lem:K3rep}
Index bonds by $k,l\in\{0,\dots,N-2\}$ and write $T_{kl}$ for the $3\times3$ block of $T$ coupling $D_k$ and $D_l$ in the
basis $(\one,t_1,t_2)$. Then $T_{kl}=\frac12(X_{kl}+X_{lk}^\top)$ with
\[
\begin{aligned}
X_{kl}={}&\frac{N-2}{2N}\,\delta_{kl}\big[(N-1-k)P_H+(k+1)P_G\big]+\one[k\le l]\,C_{HG}\\
&-\frac1N\big[(N-1-\max(k,l))C_{HH}+(\min(k,l)+1)C_{GG}+2\max(l-k,0)\,C_{HG}\big],
\end{aligned}
\]
where the six rational $3\times3$ matrices are $36P_H=\big(\begin{smallmatrix}24&-12&-12\\-12&16&-24\\-12&-24&96\end{smallmatrix}\big)$,
$36P_G=\big(\begin{smallmatrix}24&12&-12\\12&16&24\\-12&24&96\end{smallmatrix}\big)$,
$36C_{HG}=\big(\begin{smallmatrix}24&12&-12\\-12&-4&12\\-12&-12&-12\end{smallmatrix}\big)$,
$36C_{HH}=\big(\begin{smallmatrix}24&-12&-12\\-12&8&0\\-12&0&24\end{smallmatrix}\big)$,
$36C_{GG}=\big(\begin{smallmatrix}24&12&-12\\12&8&0\\-12&0&24\end{smallmatrix}\big)$: the Gram matrices, in the level
basis, of $P(J_0\,\cdot)$, $P(J_1\,\cdot)$, $\Cov(J_0\,\cdot,J_1\,\cdot)$, $\Cov(J_0\,\cdot,J_0\,\cdot)$ and
$\Cov(J_1\,\cdot,J_1\,\cdot)$ at $K=3$.
\end{lemmaS}
\begin{proof}
The three terms of \eqref{eq:formula1} contribute, respectively, the diagonal blocks $\frac{N-2}{2N}[(N-1-k)P_H+(k+1)P_G]$
(term I), the block $C_{HG}$ for $k\le l$ (term II), and, from $-\frac1N\sum_j\Var(\Omega_j)$ with
$\Omega_j=\sum_{k<j}H_k+\sum_{k\ge j}G_k$, the count of indices $j$ for which the pair $(D_k,D_l)$ enters $\Omega_j$ as
$(H,H)$, $(G,G)$ or mixed: $N-1-\max(k,l)$, $\min(k,l)+1$ and $|l-k|$ respectively. This gives the form of $X_{kl}$;
what remains is to confirm the five level matrices and the bookkeeping. To this end note that, on each of the regions
$\{k<l\}$, $\{k=l\}$, $\{k>l\}$, every entry of $N\,T_{kl}$ is a polynomial of total degree at most $2$ in $(N,k,l)$,
and so is every entry of $N$ times the Gram matrix of $K^2\fB_{N,3}$ computed directly from \eqref{eq:formula1} by
polarisation. The difference vanishes identically for $N=3,\dots,12$ (exact rational arithmetic,
\texttt{k3\_representation\_proof.py}). A polynomial of total degree at most $2$ in three variables that vanishes on the
$3\times3\times3$ grid $N\in\{7,8,9\}$, $k\in\{0,1,2\}$, $l-k\in\{1,2,3\}$---which lies inside the region $\{k<l\}$ for
every such $N$---is zero, and likewise on the $3\times3$ grid in $(N,k)$ for the diagonal region; the region $\{k>l\}$
follows by symmetry. Hence the identity holds for all $N\ge3$.
\end{proof}

\begin{lemmaS}[constant mode]\label{lem:K3u}
$T_{uu}=\frac13\big[(N-1)I-\one\one^\top\big]$ and $\one^\top T_{ur}=0$. Consequently $\fB_{N,3}\succeq0$ iff
$S:=T_{rr}-T_{ur}^\top T_{uu}^{+}T_{ur}\succeq0$, where $T_{uu}^{+}=\frac3{N-1}\big(I-\frac1{N-1}\one\one^\top\big)$; and if
$S\succ0$ then $\ker\fB_{N,3}=\operatorname{span}(\one\otimes\one)$.
\end{lemmaS}
\begin{proof}
For $D_k=u_k\one$ one has $H_k(a)=u_ka$, $G_k(a)=u_k(a+1)$, so $Z_k=0$, $\Var(D_k)=0$ and
$\mathrm{Sq}=\frac1{2N}\sum_{k<l}N(u_k-u_l)^2\Var(a)$ with $\Var(a)=\frac23$; this is
$\frac13[(N-1)\|u\|^2-(\one^\top u)^2]$. The direction $u=\one$ is $\one\otimes\one\in\ker\fB$ (proof of
Proposition~\ref{prop:T}), hence is not coupled to $r$. The rest is the Schur complement on $\one^\perp$.
\end{proof}

\begin{lemmaS}[closed forms; computer algebra]\label{lem:K3blocks}
Let $v_i=i(N-i)$ and $\Gamma_{ij}=\min(i,j)(N-\max(i,j))/N$. Then $S=\begin{pmatrix}A&B\\B^\top&C\end{pmatrix}$ with
\[
A_{ij}=\delta_{ij}\Big[\tfrac{5N-9}{36}+\tfrac{(N-2)^2v_i}{3N^2(N-1)}\Big]-\tfrac4{3N}\Gamma_{ij}-\tfrac1{36},\quad
B_{ij}=\begin{cases}\frac{(2i-N)(5N-12)}{12N}&i=j\\[2pt]\frac14-\frac j{3N}&i<j\\[2pt]\frac1{12}-\frac j{3N}&i>j\end{cases},\quad
C_{ij}=\begin{cases}\frac{5N-14}4&i=j\\[2pt]-\frac34+\frac{|i-j|}N&i\ne j.\end{cases}
\]
\end{lemmaS}
\noindent\emph{Status.} By Lemma~\ref{lem:K3rep} every entry of $T$ is, on each of the regions $\{i<j\}$, $\{i=j\}$,
$\{i>j\}$, a polynomial of degree at most $2$ in $(N,i,j)$; the Schur complement of Lemma~\ref{lem:K3u} introduces only
the sums $\sum_kT_{ur}(k,\cdot)T_{ur}(k,\cdot)$, which \texttt{s1\_closed.py} evaluates in closed form region by region
by symbolic summation, giving the formulas above as polynomial identities in $(N,i,j)$.

\paragraph{The shear.} Put $R=\operatorname{diag}\big(\frac{2i-N}{3N}\big)$, $\gamma:=\frac{N-4}2$ and
$\Theta=\begin{pmatrix}I&-R\\0&I\end{pmatrix}$. Then
\begin{equation}\label{eq:shear}
\Theta S\Theta^\top=\begin{pmatrix}\mathsf M&0\\0&C-\gamma I\end{pmatrix}
+\frac1\gamma\begin{pmatrix}\widetilde B\\\gamma I\end{pmatrix}\begin{pmatrix}\widetilde B\\\gamma I\end{pmatrix}^{\!\top},
\qquad\widetilde A=A-BR-RB^\top+RCR,\quad\widetilde B=B-RC,\quad \mathsf M:=\widetilde A-\tfrac1\gamma\widetilde B\widetilde B^\top ,
\end{equation}
which is an algebraic identity (complete the square against $\gamma I$). The shear is a congruence, not a rotation: it removes
the $O(N)$ diagonal of $B$, which couples $s_k$ and $q_k$ on the same bond; $\widetilde B_{ii}=\frac{2i-N}{6N}=O(1)$. Since
$\gamma>0$ for $N\ge5$, $S\succ0$ follows from $\mathsf M\succ0$ and $C-\gamma I\succeq0$.

\begin{lemmaS}[$C-\gamma I\succeq0$; by hand]\label{lem:K3C}
Let $z_i=\frac12-\frac iN$ and $H:=\frac2N\Gamma+2zz^\top+\frac14\one\one^\top\succeq0$. Then $C=\frac{5N-11}4I-H$ and
$\operatorname{tr}H=\frac{3(N-1)}4=\frac{5N-11}4-\gamma$. Consequently, for any factorisation $H=\sum_rh_rh_r^\top$,
\[
C-\gamma I=(\operatorname{tr}H)I-H=\sum_r\big(\|h_r\|^2I-h_rh_r^\top\big)\succeq0 .
\]
\end{lemmaS}
\begin{proof}
Off the diagonal, $\frac2N\Gamma_{ij}=\frac{2\min(i,j)}N-\frac{2ij}{N^2}$ and $2z_iz_j=\frac12-\frac{i+j}N+\frac{2ij}{N^2}$,
so $H_{ij}=\frac34-\frac{|i-j|}N=\frac{5N-11}4\delta_{ij}-C_{ij}$. On the diagonal the dependence on $i$ cancels:
$H_{ii}=\frac{2i(N-i)}{N^2}+2(\frac12-\frac iN)^2+\frac14=\frac34$. Each matrix $\|h\|^2I-hh^\top$ has eigenvalues $\|h\|^2$
and $0$.
\end{proof}

\begin{lemmaS}[$\mathsf M$ is a $Z$-matrix with positive Perron certificate; computer algebra]\label{lem:K3M}
For $i<j$, with $d=j-i$,
\[
\mathsf M_{ij}=-\frac{i(N-j)}{54N^4(N-4)}\Big[N^2(73N-423)+8N^2(N-i)+16d(N^2-d^2)+4N(i^2+j^2)+72Ni+120N(N-j)+48ij+8N+16d\Big],
\]
which is negative for $N\ge6$. Moreover
\begin{align*}
(\mathsf M\one)_i&=\frac{v_i\,\mathcal R(N,v_i)}{540N^4(N-4)(N-1)},\\
\mathcal R&=53N^5-1338N^4+5805N^3-5380N^2+384N-64\\&\quad+2(N-1)(29N^2-120N+40)v+16(N-1)v^2 ,
\end{align*}
and the substitution $N=m+19$, $v=u+(N-1)$ turns $\mathcal R$ into a polynomial in $(m,u)$ all of whose coefficients are
positive (constant term $171000$). Since $v_i-(N-1)=(i-1)(N-1-i)\ge0$, $\mathsf M\one>0$ for every $N\ge19$. For
$N=17,18$ the vector $w_i=1+\frac{(2i-N)^2}{20N^2}$ satisfies, in exact rational arithmetic,
$\min_i(\mathsf Mw)_i=\frac{7839473}{1107488460}$ and $\frac{5964113}{446410440}$ respectively.
\end{lemmaS}
\noindent\emph{Status.} The two entry formulas are polynomial identities proved by region-by-region symbolic summation
(\texttt{verify\_M\_symbolic.py}, whose hard-coded block entries are checked against \texttt{s1\_closed.py} by
\texttt{check\_blocks.py}); the positivity of the shifted coefficients and the two certificates for $N=17,18$ are exact
computations in the same script.

\begin{thmS}\label{thm:K3}
For $K=3$ and every $N\ge17$, $\fB_{N,3}\succeq0$ with kernel $\operatorname{span}(\one\otimes\one)$.
\end{thmS}
\begin{proof}
By Lemma~\ref{lem:K3M} and Lemma~\ref{lem:Zmatrix} (with $v=\one$ or $v=w$), $\mathsf M\succ0$; by Lemma~\ref{lem:K3C},
$C-\gamma I\succeq0$. In \eqref{eq:shear}, if $s\ne0$ the first block is positive on $(s,q)$, and if $s=0$, $q\ne0$ the square
term contributes $\gamma\|q\|^2>0$. Hence $\Theta S\Theta^\top\succ0$, so $S\succ0$, and Lemma~\ref{lem:K3u} concludes.
\end{proof}
The threshold is genuine for the bond form: $\lambda_{\min}(S)$ is $-0.003$ at $N=16$ and $+0.018$ at $N=17$. For $N\le16$
the bond form is indefinite on the full bond space, but it is positive on the image $\{\hat D(f)\}$, which is all that
Theorem~\ref{thm:finiteK} needs; see Step~\ref{step:certs}. The natural continuum limit of $\fB_{N,3}$ has spectral
infimum $0$, so positivity at $K=3$ is a finite-$N$ effect, which is why no continuum or Gershgorin shortcut is available.

%=====================================================================================================
\stepsection{certs}{the finitely many remaining cases (exact certificates)}\label{sec:certs}
\begin{wraptable}{r}{0.6\textwidth}\vspace{-8pt}\centering\small
\caption{Coverage of $\{(K,N):K\ge3,\ N\ge3\}$. No pair is left uncovered. The first column is analytic for $K\ge5$
(Theorem~\ref{thm:K5}) and rests on exact symbolic computation for $K=4$ and $K=3$ (Steps~\ref{step:K4}--\ref{step:K3}).}\label{tab:cov}
\begin{tabular}{@{}lcccc@{}}\toprule
$K$ & all large $N$ & bond-space certificate & image certificate & direct\\\midrule
$3$ & $N\ge17$ (Thm.~\ref{thm:K3}) & --- & $4\le N\le16$ & $N=3$\\
$4$ & $N\ge10$ (Thm.~\ref{thm:K4}) & $5\le N\le9$ & $N=3,4$ & ---\\
$5$ & $N\ge6$ (Thm.~\ref{thm:K5}) & $N=4,5$ & $N=3$ & ---\\
$6,7$ & $N\ge4$ (Thm.~\ref{thm:K5}) & $N=3$ & --- & ---\\
$\ge8$ & $N\ge3$ (Thm.~\ref{thm:K5}) & --- & --- & ---\\\bottomrule
\end{tabular}
\end{wraptable}
Theorems~\ref{thm:K5}, \ref{thm:K4} and~\ref{thm:K3} leave the pairs $(K,N)$ listed in Table~\ref{tab:cov}. They are
settled by two certificates, both in exact rational arithmetic (Python \texttt{fractions}), with no floating point.

\emph{Bond-space certificate} (\texttt{full\_space\_certificate.py}). The Gram matrix $\mathsf G$ of $\fB_{N,K}$ on
$\R^{(N-1)K}$ is built by polarisation; the script checks that $\mathsf G(\one\otimes\one)=0$ exactly and that
$\mathsf G+(\one\otimes\one)(\one\otimes\one)^\top$ has an $LDL^\top$ factorisation with positive pivots. This is equivalent
to $\fB_{N,K}\succeq0$ with kernel $\operatorname{span}(\one\otimes\one)$.

\emph{Image certificate} (\texttt{bond\_certificate.py}). Where the bond form is indefinite on the full space, the
$(N-1)\times(N-1)$ matrix of $f\mapsto\fB_{N,K}(\hat D(f))=Q^{(1)}_K+Q^{(2)}_K$ is built exactly from \eqref{eq:Dhat}. It
annihilates the linear payoff (Lemma~\ref{lem:B} and Proposition~\ref{prop:orders}), and the script certifies that it
is positive definite on the complement spanned by the second differences
$e_k-2e_{k+1}+e_{k+2}$, $k=0,\dots,N-3$, in payoff coordinates, again by $LDL^\top$ with positive pivots.

\emph{Stored certificates and an independent checker.} For each of the $25$ pairs the certified matrix $\mathsf A$
(that is, $\mathsf G+(\one\otimes\one)(\one\otimes\one)^\top$, respectively the image matrix), the unit lower-triangular
factor $\mathsf L$ and the pivots $\mathsf D$ are stored as exact rationals in \texttt{certificates/*.json}
(\texttt{make\_certificates.py}). The checker \texttt{verify\_certificates.py} uses only the Python standard library
and imports none of the code that produced them. For every file it (1)~rebuilds $\mathsf A$ from
\eqref{eq:formula1} and \eqref{eq:Dhat}---an implementation independent of the generator, which evaluates the bond form
through the bridge kernels of the original proof notes---and checks equality entry by entry; (2)~checks that
$\mathsf L$ is unit lower triangular, that all pivots are positive and that $\mathsf L\mathsf D\mathsf L^\top=\mathsf A$
exactly; and (3)~checks the kernel statement ($\mathsf G(\one\otimes\one)=0$, respectively that the bond vectors of the
linear payoff pair to zero with everything). A reader who trusts rational arithmetic therefore needs to trust only
this one short file, together with Proposition~\ref{prop:bond} (which identifies $\fB_{N,K}(\hat D(f))$ with
$Q^{(1)}_K+Q^{(2)}_K$) and Proposition~\ref{prop:orders}. All $25$ certificates pass.

\emph{The pair $(K,N)=(3,3)$.} Here the two-body form vanishes identically on the image, and we compute $Q_3$ itself in
exact arithmetic from the definition: $Q_3=\frac83\begin{pmatrix}1&-1\\-1&1\end{pmatrix}$, positive semidefinite with kernel
$\operatorname{span}(\one)$ (generalised eigenvalue $\frac{32/3}{36}=\frac8{27}$).

\noindent The log of the certificate run contains four lines reporting that the \emph{bond-space} certificate fails, at
$(K,N)=(3,3),(4,3),(4,4),(5,3)$. These are expected: there the bond form is indefinite (or degenerate) on the full space,
and the pairs are covered by the image certificate or, for $(3,3)$, directly. The annotated log marks them accordingly.

%=====================================================================================================
\stepsection{assembly}{assembly, the case \texorpdfstring{$N=2$}{N=2}, and \texorpdfstring{$K=2$}{K=2}}\label{sec:assembly}
Everything is now in place: the orders $m\ge3$ (Step~\ref{step:orders}), the two-body form on the bond space (Steps~\ref{step:bond}--\ref{step:certs}), and
the kernel (Steps~\ref{step:B} and~\ref{step:kerSq}). The case $N=2$ is trivial.
\begin{proof}[Proof of Theorem~\ref{thm:finiteK}]
Let $K\ge3$. \emph{$N=2$.} The increment space is one-dimensional and spanned by $\one$, so $Q_K=0$ by
Lemma~\ref{lem:B}, and the statement is trivial (every non-constant $f$ is affine). \emph{$N\ge3$.} By
Lemma~\ref{lem:orderdec}, $F^\top Q_KF=K^{N+1}\sum_{m\ge1}Q^{(m)}_K(f)$; by Proposition~\ref{prop:orders},
$Q^{(m)}_K\succeq0$ for $m\ge3$; by Proposition~\ref{thm:C}, $Q^{(1)}_K+Q^{(2)}_K=\fB_{N,K}(\hat D(f))$. By
Theorems~\ref{thm:K5}, \ref{thm:K4}, \ref{thm:K3} and Table~\ref{tab:cov}, this is nonnegative for every $f$, so
$Q_K\succeq0$. For the kernel, $\one\in\ker Q_K$ by Lemma~\ref{lem:B}. Conversely let $F^\top Q_KF=0$. Every summand
vanishes, in particular $\fB_{N,K}(\hat D(f))=0$. In the large-$N$ and bond-space cases
$\ker\fB_{N,K}=\operatorname{span}(\one\otimes\one)$, so $f$ is affine by Lemma~\ref{lem:transfer}; in the image-certified
cases the form is positive definite on a complement of the linear payoff, so $f$ is affine; and $(3,3)$ was computed
directly.
\end{proof}

\paragraph{Where $K\ge3$ enters, and the counterexample at $K=2$.} Proposition~\ref{thm:C} and Theorem~\ref{thm:SOS} hold for
$K=2$. The hypothesis enters through Lemma~\ref{lem:Lstar-SM} alone: its margin $(K-2)\mu\nu\Var(D)$ vanishes
identically for binary priorities, and every later step inherits this. Correspondingly the statement is false at $K=2$:
building $Q_2$ at $N=7$ from the definition in exact rational arithmetic (\texttt{k2\_witness.py}), the strictly decreasing
payoff with increments $F=(9,8,6,4,2,1)$ gives
\[
F^\top Q_2F=-\frac{7237}{480}<0,\qquad\rho_\pot=\frac{53454277}{62354880}>\frac67 ,
\]
and the reversed increments give the same values. For $N\le6$, $Q_2\succeq0$. Table~\ref{tab:gap-SM} records the
margin $\frac{N-1}N-\max_f\rho_\pot(f)$ over non-affine $f$ for small $(K,N)$: it is positive throughout $K\ge3$, in
agreement with Theorem~\ref{thm:finiteK}, turns negative at $K=2$ exactly at $N=7$, and grows in magnitude with $N$.

\begin{table}[htbp]\centering
\caption{Margin $\frac{N-1}N-\max_f\rho_\pot(f)$ over non-affine payoff-from-rank functions $f$ on $K_N$, computed
in floating point from the pencil $(M_\pot,M_{\mathrm{tot}})$ (not part of any proof). When positive it is the gap
$\lambda_1-\lambda_2$ between the two largest generalised eigenvalues, and as $K\to\infty$ it tends to
$\lambda_1-\lambda_2=\frac2{N+2}$ of Theorem~\ref{thm:spectrum}. The entries at $K=2$, $N\ge7$ (bold) are negative,
in agreement with the exact witness at $N=7$; blank cells were not computed.}\label{tab:gap-SM}
\small
\begin{tabular}{@{}rccccccc@{}}\toprule
$N$ & $K=2$ & $K=3$ & $K=4$ & $K=5$ & $K=6$ & $K=7$ & $K=8$\\\midrule
3  & $+.167$ & $+.296$ & $+.342$ & $+.363$ & $+.374$ & $+.381$ & $+.385$\\
4  & $+.075$ & $+.216$ & $+.267$ & $+.291$ & $+.304$ & $+.311$ & $+.317$\\
5  & $+.033$ & $+.169$ & $+.219$ & $+.243$ & $+.256$ & $+.264$ & $+.269$\\
6  & $+.011$ & $+.138$ & $+.186$ & $+.209$ & $+.221$ & $+.229$ & $+.234$\\
7  & $\mathbf{-.001}$ & $+.116$ & $+.161$ & $+.183$ & $+.195$ & $+.202$ & $+.207$\\
8  & $\mathbf{-.009}$ & $+.100$ & $+.142$ & $+.163$ & $+.174$ & $+.181$ & $+.185$\\
9  & $\mathbf{-.014}$ & $+.088$ & $+.127$ & $+.147$ & $+.157$ & & \\
10 & $\mathbf{-.017}$ & $+.078$ & $+.115$ & & & & \\
11 & $\mathbf{-.019}$ & $+.070$ & & & & & \\
12 & $\mathbf{-.020}$ & $+.063$ & & & & & \\\bottomrule
\end{tabular}
\end{table}


%=====================================================================================================
\subsection{The reciprocity law: proof of Proposition~\ref{prop:recip}}\label{sec:recip}
This subsection is independent of Steps~\ref{step:hoeff}--\ref{step:assembly}. It does not give another proof of Theorem~\ref{thm:finiteK}; it
describes exactly how the finite-$K$ forms deviate from the continuum ones.

\paragraph{Setting.} $C=([N],E)$ is a conflict graph and the protocol is given by a total order $\prec$ of the agents:
$j$ is served before its neighbour $i$ iff $s_j>s_i$, or $s_j=s_i$ and $j\prec i$; $\prec^{\rm rev}$ is the reversed
order. For $S\subseteq[N]$ put $A_S=\prod_{j\in S}A_j$. With $u_i=f(\pos_C(i,\cdot))$, $g_i=(I-A_i)u_i$ and $g=\sum_ig_i$,
the forms
\[
\mathsf m_{\rm tot}(f,f')=\sum_i\E\big[g_i^{f}g_i^{f'}\big],\qquad
\mathsf m_{\pot}(f,f')=\E\big[g^{f}\,\numop^{-1}g^{f'}\big]
\]
are $K^{-(N+1)}$ times the two energy forms, and $K^{-(N+1)}Q_K=\frac{N-1}N\mathsf m_{\rm tot}-\mathsf m_\pot$ on $K_N$. We write
$\mathsf m^{\prec}(K)$ for either of them, as a function of $K$.

\begin{mainthm}[Proposition~\ref{prop:recip} of the main text]
{\rm(a)} $\mathsf m^{\prec}(K)$ is a polynomial in $1/K$ of degree at most $2N-1$; its constant term is the
corresponding form of the game with continuous priorities on $C$. {\rm(b)} As polynomials in $x=1/K$,
$\mathsf m^{\prec}(-x)=\mathsf m^{\prec^{\rm rev}}(x)$. {\rm(c)} If $C$ has an automorphism $\pi$ with
$\pi(j)\prec\pi(i)$ whenever $\{i,j\}\in E$ and $i\prec j$, then $\mathsf m^{\prec}(K)$ is a polynomial in $K^{-2}$ of
degree at most $N-1$ that vanishes at $K=1$.
\end{mainthm}

\emph{(1) Reduction to counting.} Let $U^r_i=\one[\pos_C(i,\cdot)=r]$, so that $u_i=\sum_rf(r)U_i^r$. The $A_j$
are commuting orthogonal projections, so
$\prod_{j\in T}(I-A_j)\prod_{j\notin T}A_j=\sum_{S\supseteq T^c}(-1)^{|S\setminus T^c|}A_S$, and $\numop^{-1}$ acts on the
range of this projection as $1/|T|$ (Lemma~\ref{lem:numop}). Hence both forms are linear combinations, with
coefficients that do not depend on $K$, of
\[
F(K)=\E\big[U_i^{r}\cdot A_SU_k^{r'}\big],\qquad i,k\in[N],\ S\subseteq[N]
\]
(the projections $I-A_i$ in $g_i$ are absorbed into $S$, since $A_SA_i=A_{S\cup\{i\}}$). Now
$A_SU_k^{r'}(s)=\E'[U_k^{r'}(s')]$, where $s'_j=s_j$ for $j\notin S$ and the $s'_j$, $j\in S$, are fresh independent
uniform levels. With $n=N+|S|\le2N$,
\begin{equation}\label{eq:count}
F(K)=K^{-n}\,\#\big\{(s,s'_S)\in\{0,\dots,K-1\}^n:\ \pos(i,s)=r,\ \pos(k,s')=r'\big\}.
\end{equation}

\emph{(2) Lexicographic cells.} Order the $n$ coordinates by the agent they belong to, according to $\prec$,
and put $s_j$ before its twin $s'_j$; call this total order of the coordinates $\prec$ again. The rule for twins is an
auxiliary choice: any other rule gives another decomposition of the same set into cells, and
\eqref{eq:Fcells} below holds for each of them. Every point of the cube induces a strict
total order $\sigma$ of the coordinates: larger level first, ties broken by $\prec$. The set in \eqref{eq:count} is a
union of such cells: $\pos(i,s)$ is the number of neighbours of $i$ that precede $s_i$ in $\sigma$, and likewise for
$\pos(k,s')$; only coordinates of \emph{different} agents are ever compared, so the convention for twins is immaterial.
Let $\mathcal O$ be the set of orders $\sigma$ for which the two conditions hold. \emph{It is defined without reference
to the protocol.}

\begin{lemmaS}[cells]\label{lem:cells}
For a strict order $\sigma=(\sigma_1,\dots,\sigma_n)$ let
$\operatorname{des}_\prec(\sigma)=\#\{t:\sigma_{t+1}\prec\sigma_t\}$. The number of points of $\{0,\dots,K-1\}^n$ whose
lexicographic order is $\sigma$ equals $\binom{K+n-1-\operatorname{des}_\prec(\sigma)}n$.
\end{lemmaS}
\begin{proof}
The levels $v_t$ of $\sigma_t$ satisfy $v_1\ge\dots\ge v_n$, with $v_t>v_{t+1}$ required exactly when
$\sigma_{t+1}\prec\sigma_t$ (a tie would have put $\sigma_{t+1}$ first). Subtracting from $v_t$ the number of forced
strict steps at positions $\ge t$ gives a bijection with the weakly decreasing sequences in
$\{0,\dots,K-1-\operatorname{des}_\prec(\sigma)\}$, of which there are $\binom{K-\operatorname{des}_\prec(\sigma)+n-1}n$.
\end{proof}
\noindent Therefore
\begin{equation}\label{eq:Fcells}
F^{\prec}(K)=K^{-n}\sum_{\sigma\in\mathcal O}\binom{K+n-1-\operatorname{des}_\prec(\sigma)}n .
\end{equation}
Each binomial is a polynomial of degree $n$ in $K$ divisible by $K$, since $0\le n-1-\operatorname{des}\le n-1$. Hence
$F$ is a polynomial in $1/K$ of degree at most $n-1\le2N-1$, with constant term $|\mathcal O|/n!$, which is the
probability that $n$ i.i.d.\ continuous priorities fall in $\mathcal O$, i.e.\ the value of $F$ in the continuum game.
This proves (a).

\emph{(3) Reciprocity.} For integers $n\ge1$ and $d$, $\binom{-K+n-1-d}{n}=(-1)^n\binom{K+d}{n}$ as polynomials
in $K$. Let $\prec^{\rm rev}$ denote the reversal of the \emph{whole} order of the $n$ coordinates, twins included. Since
$\prec$ is a total order, every adjacent pair of $\sigma$ is either a descent or an ascent, so
$n-1-\operatorname{des}_\prec(\sigma)=\operatorname{des}_{\prec^{\rm rev}}(\sigma)$. (Reversing the order of the agents
but not that of the twins would break this identity whenever two twins are adjacent in $\sigma$.) On coordinates of
different agents $\prec^{\rm rev}$ is the reversed protocol, and by (2) its rule for twins is immaterial, so the
right-hand side of \eqref{eq:Fcells} written for $\prec^{\rm rev}$ is $F$ for the game with the reversed protocol. Substituting in \eqref{eq:Fcells},
\[
F^{\prec}(-K)=(-K)^{-n}(-1)^n\sum_{\sigma\in\mathcal O}\binom{K+\operatorname{des}_\prec(\sigma)}{n}
=K^{-n}\sum_{\sigma\in\mathcal O}\binom{K+n-1-\operatorname{des}_{\prec^{\rm rev}}(\sigma)}{n}=F^{\prec^{\rm rev}}(K),
\]
because $\mathcal O$ is the same set for both protocols. This is an instance of the reciprocity theorem for
$P$-partitions \cite[Sec.~3.15.3]{stanley2012}, equivalently of Ehrhart--Macdonald reciprocity for order polytopes:
changing the sign of the dilation exchanges weak and strict inequalities, that is, it exchanges who wins a tie. Summing
with the $K$-independent coefficients of (1) gives (b).

\emph{(4) Symmetric protocols.} If $\pi$ is as in (c), relabelling the agents by $\pi$ maps the game with
protocol $\prec^{\rm rev}$ onto the game with protocol $\prec$ on the same graph, and the forms, being sums over all
agents, are invariant. Hence $\mathsf m^{\prec^{\rm rev}}=\mathsf m^{\prec}$, and (b) shows that $\mathsf m^{\prec}$ is
even in $1/K$; being of degree at most $2N-1$, it has degree at most $2N-2$. At $K=1$ every $g_i$ vanishes, and
\eqref{eq:Fcells} holds for every integer $K\ge1$, so the polynomial vanishes at $K=1$. On $K_N$ the reversal
$i\mapsto N-1-i$ is such an automorphism, which gives \eqref{eq:Qexpansion}. \qed

\noindent\emph{What the expansion does not say.} It concerns the forms, not their eigenvalues. At finite $K$ the order
forms do not commute, and the generalised eigenvalues are algebraic functions of $y=K^{-2}$, not polynomials. Because
the continuum eigenvalues $\lambda_p$ are simple (Theorem~\ref{thm:spectrum}), analytic perturbation theory applies
at $y=0$: the finite-$K$ eigenvalues are analytic in $y$ near $0$, hence equal to $\lambda_p+O(K^{-2})$, with no term
of order $K^{-1}$. Whether the coefficient of $K^{-2}$ is non-zero for a given $p$ is not claimed.

\begin{remarkS}[tests of the reciprocity law]
By (b), when no automorphism reverses the protocol the expansions for $\prec$ and $\prec^{\rm rev}$ have equal even
and opposite odd coefficients: on the star with a favoured centre ($N=4$, prize table $(0,-1,-3,-4.5)$) the term
$-0.5625K^{-1}$ of $\mathsf m_\pot$ changes sign under relabelling while $2.1043-2.5085K^{-2}$ does not, and the same
holds on the path $0$--$1$--$3$--$2$ and the paw graph to $10^{-7}$; on $K_4$ the odd coefficients vanish.
\end{remarkS}

\begin{remarkS}[the critical number of levels; what survives at finite $K$]
The numbers $K^\star(N)$ quoted in Remark~\ref{rem:K2} are obtained by interpolating exact enumerations of $Q_K$ in
$y=K^{-2}$ (for $N\le6$ the fit is over-determined, with residuals below $10^{-13}$). The same computations show, for
$N\le7$, that in the discrete Chebyshev basis all forms split by the parity of the degree, that the order-$m$ potential
form vanishes on polynomials of degree less than $m$, and that the order forms do \emph{not} commute at finite $K$: the
order-by-order diagonalisation of Theorem~\ref{thm:spectrum} is a property of the continuum. The proof above requires
a total-order protocol; orientations with directed cycles and randomised tie-breaking are not covered.
\end{remarkS}

\section{The harmonic component of the linear game: tie-pattern law and randomised tie-breaking}\label{sec:pattern}
Throughout this appendix the game is the linear rank-order game $\calG(C,K)$ on an arbitrary conflict graph $C$. By
Proposition~\ref{prop:hflow}, along an edge $(i,s\to s')$ the harmonic flow is $h(i,s\to s')=W-d_i\ell/K$, the
deviation of the number $W$ of overtaken neighbours from its mean under uniformly random levels. Define the harmonic
energy of a profile as
\[
H(s):=\sum_i\sum_{s'_i>s_i}h(i,s\to s')^2 ,
\]
so that $\Eharm=\sum_sH(s)=K^N\,\E[H]$: $H$ assigns the energy of every edge of the game graph to its lower
endpoint. $H(s)$ depends on this convention and on the tie-breaking order, and should not be read as a dissipation at
$s$. Let $\bar H$ be the average of $H$ over a uniformly random total order of the agents used
as the protocol. The deviation $h$ is produced most strongly by ties, and the following theorem makes this exact: the
conditional expectation of $\bar H$ given the tie pattern is an explicit linear function of the pattern.

\begin{thmS}[tie-pattern law]\label{thm:pattern-SM}
Let $\tau_{jk}=\one[s_j=s_k]$, $e_{jk}=\one[\{j,k\}\in E]$,
$c_{jk}=|\calN(j)\cap \calN(k)|$, and let $\bar H_i$ be the harmonic energy of
player~$i$ averaged over a uniformly random tie-breaking order,
$\bar H=\sum_i\bar H_i$. Then for every player~$i$
\begin{equation}\label{eq:perplayer}
\E[\bar H_i\mid\tau]=\frac{K-1}6\sum_{\{j,k\}\subseteq \calN(i)}\tau_{jk}
+\frac{K-2}{12}\sum_{j\in \calN(i)}\tau_{ij}+\mathsf c_i,\quad
\mathsf c_i=\frac{d_i\big[K^2-K+1-(d_i-1)(K-1)\big]}{12K},
\end{equation}
and summing over $i$,
$\E[\bar H\mid\tau]=\calA_C(s)+\mathsf c_C$, where
$\calA_C(s)=\sum_{j<k}\big[\frac{K-2}6e_{jk}+\frac{K-1}6c_{jk}\big]\tau_{jk}$ is the weighted tie count
with $\mathsf c_C=\sum_i\mathsf c_i=\frac{K^2-1}{12K}\sum_id_i-\frac1K\big[\frac{K-2}6|E|+\frac{K-1}6\sum_i\binom{d_i}2\big]$.
\end{thmS}

\begin{proof}
\emph{(0) Localisation.} By Proposition~\ref{prop:hflow}, $h(i,s\to s')=W-d_i\ell/K$
depends on $s$ only through $s|_{\{i\}\cup \calN(i)}$ and on the tie-breaking
order only through its restriction to $\{i\}\cup \calN(i)$. Conditionally on
the global tie pattern $\tau$, the levels of the tie classes are a
uniformly random injective assignment of $\{0,\dots,K-1\}$ to the classes;
its restriction to $\{i\}\cup \calN(i)$ is again a uniformly random injective
assignment to the local classes. Hence $\E[\bar H_i\mid\tau]$ depends only
on $\tau|_{\{i\}\cup \calN(i)}$. Fix $i$, write $b=s_i$, and let $\mathcal T_i$ be the tie class of~$i$ (the players at level~$b$).

\emph{(1) Two-body form.} For a target level $a>b$ and a neighbour
$j$ let $I_j=\one[b<s_j<a]+\one[s_j=b,\,j\prec i]+\one[s_j=a,\,i\prec j]$,
where $\prec$ is the random order, so that $W=\sum_jI_j$. For uniform
$s_j$ and uniform order, $\E I_j=\ell/K=:\bar\ell$ with $\ell=a-b$, hence
$d_i\ell/K=\sum_j\bar\ell$ and
\[
\bar H_i=\sum_{a>b}\E_\prec\Big[\Big(\sum_j(I_j-\bar\ell)\Big)^2\Big]
=\sum_{a>b}\Big[\sum_j\E_\prec(I_j-\bar\ell)^2+\sum_{j\ne k}\E_\prec(I_j-\bar\ell)(I_k-\bar\ell)\Big].
\]
The kernels do not depend on~$d_i$.

\emph{(2) Types.} For fixed $b$, $\E_\prec[\cdot]$ depends on
$s_j,s_k$ only through their position relative to $(b,a)$ and on the
order of $\{i,j,k\}$. Taking the expectation over the levels given the
local pattern, the one-body term depends only on whether $j\sim i$
(constants $\varpi_1^{\mathrm t}$, $\varpi_1^{\mathrm f}$), and the two-body term only on the
pattern type of $\{i,j,k\}$: all distinct ($\varpi_{\rm dist}$),
$j\sim k\not\sim i$ ($\varpi_{\rm pair}$), exactly one of $j,k$ tied with $i$
($\varpi_{\rm one}$; the two cases are equal by symmetry), all tied
($\varpi_{\rm all}$).

\emph{(3) Counting.} Let $n_t=|\mathcal T_i\cap \calN(i)|$ be the number of neighbours tied with~$i$ and
$n_c=\sum_{\mathcal T\ne\mathcal T_i}\binom{|\mathcal T\cap \calN(i)|}2$, the sum running over
the other tie classes~$\mathcal T$, the number of
tied neighbour pairs not involving~$i$. Ordered neighbour pairs $(j,k)$
fall into the types with multiplicities $n_t(n_t-1)$ (all tied),
$2n_t(d_i-n_t)$ (one tied with $i$), $2n_c$ ($j\sim k\not\sim i$) and
$(d_i-n_t)(d_i-n_t-1)-2n_c$ (distinct). Hence
\begin{align*}
\E[\bar H_i\mid\tau]&=n_t\varpi_1^{\mathrm t}+(d_i-n_t)\varpi_1^{\mathrm f}+n_t(n_t-1)\varpi_{\rm all}
+2n_t(d_i-n_t)\varpi_{\rm one}\\
&\quad+2n_c\,\varpi_{\rm pair}+\big[(d_i-n_t)(d_i-n_t-1)-2n_c\big]\varpi_{\rm dist}\\
&=2(\varpi_{\rm pair}-\varpi_{\rm dist})\,n_c+2(\varpi_{\rm all}-2\varpi_{\rm one}+\varpi_{\rm dist})\tbinom{n_t}2\\
&\quad+\big[\varpi_1^{\mathrm t}-\varpi_1^{\mathrm f}+2(d_i-1)(\varpi_{\rm one}-\varpi_{\rm dist})\big]\,n_t\\
&\quad+d_i\varpi_1^{\mathrm f}+d_i(d_i-1)\varpi_{\rm dist}.
\end{align*}
Note $\sum_{\{j,k\}\subseteq \calN(i)}\tau_{jk}=\binom{n_t}2+n_c$ and
$\sum_{j\in \calN(i)}\tau_{ij}=n_t$.

\emph{(4) The six constants.} Fix $b=s_i$, a target $a>b$,
$\ell=a-b$ and $\bar\ell=\ell/K$. Given the levels of $j$ and $k$, the random order
enters only through the events $j\prec i$, $i\prec k$, etc., whose
probabilities are $\frac12$ for one comparison and $\frac13$ (same
side) or $\frac16$ (opposite sides) for two comparisons involving~$i$.
Hence, with $I_j=\one[b<s_j<a]+\one[s_j=b]\one[j\prec i]+\one[s_j=a]\one[i\prec j]$,
\[
\E_\prec(I_j-\bar\ell)^2=\begin{cases}(1-\bar\ell)^2 & b<s_j<a,\\[2pt]
\tfrac12\big[(1-\bar\ell)^2+\bar\ell^2\big] & s_j\in\{b,a\},\\[2pt]
\bar\ell^2 & \text{otherwise},\end{cases}
\]
and, writing $\epsilon_j\in\{1,\tfrac12,0\}$ for $\E_\prec I_j$ according
to whether $s_j$ lies strictly between, on $\{b,a\}$, or elsewhere,
\[
\E_\prec(I_j-\bar\ell)(I_k-\bar\ell)=(\epsilon_j-\bar\ell)(\epsilon_k-\bar\ell)+\zeta_{jk},\qquad
\zeta_{jk}=\begin{cases}\tfrac1{12} & s_j=s_k\in\{b,a\},\\[2pt]
-\tfrac1{12} & \{s_j,s_k\}=\{b,a\},\\[2pt]
0 & \text{otherwise}\end{cases}
\]
(the correction $\zeta$ is the covariance of the two order indicators:
$\frac13-\frac14$ when both compare with $i$ from the same side,
$\frac16-\frac14$ from opposite sides). Each constant is now an average
of these expressions over $b$ uniform, $a>b$, and the levels of the
other players consistent with the type: a level tied with $i$ is~$b$;
a free level is uniform on the $K-1$ values $\ne b$; two free untied
levels are uniform on distinct pairs. Counting the levels by region
($b$ below, $\ell-1$ strictly between, one at $a$, $K-1-a$ above) turns
each average into a polynomial in $b,\ell$ which is then summed over
$0\le b<a\le K-1$; the summations are elementary (Faulhaber) and give
\begin{equation}\label{eq:consts}
\begin{gathered}
\varpi_1^{\mathrm f}=\frac{K^2-K+1}{12K},\qquad
\varpi_1^{\mathrm t}=\frac{(2K-1)(K-1)}{12K},\\[2pt]
\varpi_{\rm dist}=\varpi_{\rm one}=-\frac{K-1}{12K},\qquad
\varpi_{\rm pair}=\varpi_{\rm all}=\frac{(K-1)^2}{12K},\\[2pt]
\text{so that}\quad
\varpi_{\rm one}-\varpi_{\rm dist}=0,\qquad
\varpi_{\rm pair}-\varpi_{\rm dist}=\varpi_{\rm all}-\varpi_{\rm dist}=\frac{K-1}{12},\qquad
\varpi_1^{\mathrm t}-\varpi_1^{\mathrm f}=\frac{K-2}{12}.
\end{gathered}
\end{equation}
For instance, $\varpi_1^{\mathrm f}$ is
$\frac1{K(K-1)}\sum_{b<a}\big[(\ell-1)(1-\bar\ell)^2+\tfrac12\big((1-\bar\ell)^2+\bar\ell^2\big)+(K-1-\ell)\bar\ell^2\big]$
and $\varpi_1^{\mathrm t}=\frac1K\sum_{b<a}\tfrac12\big[(1-\bar\ell)^2+\bar\ell^2\big]$.

\emph{(4a) The four two-body constants, in full.} The identity
$\varpi_{\rm one}=\varpi_{\rm dist}$ carries the theorem, so this part of the
computation is given in detail. Fix $b$ and $a>b$, put $\ell=a-b$,
$\bar\ell=\ell/K$ and $\delta:=\tfrac12-\bar\ell$, and set, for a level
$v\in\{0,\dots,K-1\}$,
\[
\epsilon(v)=\begin{cases}1,&b<v<a,\\[1pt] \tfrac12,& v\in\{b,a\},\\[1pt] 0,&\text{otherwise,}\end{cases}
\qquad \Phi(v):=\epsilon(v)-\bar\ell ,
\]
so that $\E_\prec I_j=\epsilon(s_j)$ and $\Phi(b)=\Phi(a)=\delta$. Two
identities drive the whole step. First, since
$\sum_v\epsilon(v)=(\ell-1)+\tfrac12+\tfrac12=\ell=K\bar\ell$,
\begin{equation}\label{eq:Phizero}
\sum_{v=0}^{K-1}\Phi(v)=0,\qquad\text{hence}\qquad \sum_{v\ne b}\Phi(v)=-\delta .
\end{equation}
Second, with $E_2:=\sum_v\Phi(v)^2=(\ell-1)(1-\bar\ell)^2+2\delta^2+(K-\ell-1)\bar\ell^2$,
\begin{equation}\label{eq:E2id}
E_2-K\delta^2=\frac{2\ell(K-\ell)}K-\frac{K+2}4 .
\end{equation}
Indeed, writing $m=K-\ell$,
$(\ell-1)m^2+(m-1)\ell^2=K\ell m-(\ell^2+m^2)=(K+2)\ell m-K^2$ and
$(K-2\ell)^2=(m-\ell)^2=K^2-4\ell m$, so that
$K^2\big(E_2-K\delta^2\big)=(K+2)\ell m-K^2-\tfrac{K-2}4\big(K^2-4\ell m\big)=2K\ell m-\tfrac{K+2}4K^2$.

Now average $\E_\prec(I_j-\bar\ell)(I_k-\bar\ell)=\Phi(s_j)\Phi(s_k)+\zeta_{jk}$
over the levels admitted by each type (a level tied with $i$ equals $b$; a
free level is uniform on the $K-1$ values $\ne b$; two free untied levels
are uniform on the ordered distinct pairs among those $K-1$ values). The
$\zeta$ term contributes $+\tfrac1{12}$ exactly when $s_j=s_k\in\{b,a\}$ and
$-\tfrac1{12}$ exactly when $\{s_j,s_k\}=\{b,a\}$; in the ``one tied'' type
this requires $s_k=a$, of probability $\tfrac1{K-1}$, and in the ``all
distinct'' type it cannot occur, since neither level equals~$b$. Using
\eqref{eq:Phizero} and $\sum_{v\ne b}\Phi(v)^2=E_2-\delta^2$,
\begin{equation}\label{eq:types}
\begin{aligned}
\text{all tied}&:&& \delta^2+\tfrac1{12},\\
\text{exactly one tied with }i&:&& \frac{\delta}{K-1}\sum_{v\ne b}\Phi(v)-\frac1{12(K-1)}
   =-\frac{\delta^2+\tfrac1{12}}{K-1},\\
j\sim k\not\sim i&:&& \frac{E_2-\delta^2}{K-1}+\frac1{12(K-1)},\\
\text{all distinct}&:&& \frac{\big(\sum_{v\ne b}\Phi(v)\big)^2-\sum_{v\ne b}\Phi(v)^2}{(K-1)(K-2)}
   =\frac{2\delta^2-E_2}{(K-1)(K-2)} .
\end{aligned}
\end{equation}
Each constant is $\frac1K\sum_{0\le b<a\le K-1}$ of the corresponding line of
\eqref{eq:types}. Since $\delta=\frac{K-2\ell}{2K}$ and $E_2$ depend on
$(b,a)$ only through $\ell$, which occurs with multiplicity $K-\ell$, and
since $\sum_{\ell=1}^{K-1}\ell(K-\ell)^2=\frac{K^2(K^2-1)}{12}$,
\begin{equation}\label{eq:faul}
\sum_{b<a}1=\binom K2,\quad
\sum_{b<a}\delta^2=\frac{(K-1)(K-2)}{24},\quad
\sum_{b<a}\!\big(E_2-K\delta^2\big)=\frac{K(K-1)(K-2)}{24},
\end{equation}
the last by \eqref{eq:E2id}, whence $\sum_{b<a}E_2=\frac{K(K-1)(K-2)}{12}$.
Substituting \eqref{eq:faul} into \eqref{eq:types} gives the four values
in \eqref{eq:consts}.

The two coincidences in \eqref{eq:consts} are one identity, not two. Put
\[
\Theta:=\sum_{0\le b<a\le K-1}\Big[E_2-K\delta^2-\frac{K-2}{12}\Big].
\]
Subtracting the lines of \eqref{eq:types} termwise,
\[
\varpi_{\rm one}-\varpi_{\rm dist}=\frac{\Theta}{K(K-1)(K-2)},\qquad
\varpi_{\rm pair}-\varpi_{\rm all}=\frac{\Theta}{K(K-1)},
\]
and by \eqref{eq:faul}, $\Theta=\frac{K(K-1)(K-2)}{24}-\frac{K-2}{12}\binom K2=0$.
Equivalently, by \eqref{eq:E2id} the summand of $\Theta$ is
$\frac{2\ell(K-\ell)}K-\frac{K+1}3$, and
$\frac2K\sum_\ell\ell(K-\ell)^2=\frac{K(K-1)(K+1)}6=\frac{K+1}3\binom K2$.
Hence $\varpi_{\rm one}=\varpi_{\rm dist}$ and $\varpi_{\rm pair}=\varpi_{\rm all}$:
the first removes the $d_i$-dependence of the $n_t$ coefficient in (3),
the second merges $\binom{n_t}2$ and $n_c$ into the single statistic
$\sum_{\{j,k\}\subseteq\calN(i)}\tau_{jk}$.

Substituting \eqref{eq:consts} into (3):
the coefficient of $n_c$ is $\frac{K-1}6$; the coefficient of
$\binom{n_t}2$ is $\frac{K-1}6$ as well, so the two combine into
$\frac{K-1}6\sum_{\{j,k\}\subseteq \calN(i)}\tau_{jk}$; the coefficient of
$n_t$ is $\varpi_1^{\mathrm t}-\varpi_1^{\mathrm f}=\frac{K-2}{12}$, since $\varpi_{\rm one}=\varpi_{\rm dist}$; the constant is $\mathsf c_i=d_i\varpi_1^{\mathrm f}+d_i(d_i-1)\varpi_{\rm dist}$.
The identity $\varpi_{\rm one}=\varpi_{\rm dist}$ is what removes the
$d_i$-dependence of the $n_t$ coefficient. This proves
\eqref{eq:perplayer}.

\emph{(5) Summation.} A tied pair $\{j,k\}$ contributes
$\frac{K-2}{12}$ to $\bar H_j$ and to $\bar H_k$ if $\{j,k\}\in E$, and
$\frac{K-1}6$ to $\bar H_i$ for every common neighbour~$i$. Finally
$\E[\bar H_i]=\mathsf c_i+\frac{K-1}6\binom{d_i}2\frac1K+\frac{K-2}{12}\frac{d_i}K
=\frac{d_i(K^2-1)}{12K}$ gives
$\mathsf c_C=\frac{K^2-1}{12K}\sum_id_i-\frac1K\big[\frac{K-2}6|E|+\frac{K-1}6\sum_i\binom{d_i}2\big]$.
\end{proof}

\begin{corS}[complete graph]\label{cor:law-SM}
On $K_N$, with $A(s)$ the number of tied pairs, $\E[H\mid A=a]=c_1a+c_0$ for the index protocol, where
$c_1=\frac{(K-1)N-K}6$ and $c_0=\frac{N(N-1)[K^2+K-1-(K-1)N]}{12K}$.
\end{corS}
\begin{proof}
On $K_N$ every pair is an edge with $N-2$ common neighbours, so the
weight of every tied pair is
$\frac{K-2}6+(N-2)\frac{K-1}6=\frac{(K-1)N-K}6=c_1$, and Theorem~\ref{thm:pattern-SM}
gives $\E[\bar H\mid\tau]=c_1A(s)+c_0$ with $A=\sum_{j<k}\tau_{jk}$
and $c_0=\mathsf c_{K_N}=\frac{N(N-1)[K^2+K-1-(K-1)N]}{12K}$ (a direct
simplification). Conditioning on $A$ and using the tower property gives
$\E[\bar H\mid A=a]=c_1a+c_0$. It remains to replace $\bar H$ by the
fixed-order energy $H$: for a permutation $\sigma$ of the players,
$H(\sigma s)$ is the energy of the game with tie-breaking order
$\sigma$; since the law of $s$ given $A$ is exchangeable in the players,
$\E[H\mid A]=\E[H\circ\sigma\mid A]$ for every $\sigma$, hence
$\E[H\mid A]=\E[\bar H\mid A]$.
\end{proof}



\begin{figure}[htbp]\centering
\includegraphics[width=0.8\textwidth]{figs/fig3_harmonic_law.pdf}
\caption{The tie-pattern law against exhaustive enumeration (floating point; not part of any proof).
(a)~Complete graph, index protocol: $\E[H\mid A]$ against the number $A$ of tied pairs (points) and the affine law of
Corollary~\ref{cor:law-SM} (lines).
(b)~$C_4$, $P_4$, $S_4$, $K=3$: the order-averaged energy $\E[\bar H\mid\calA_C]$ lies on the line of slope one given by
\eqref{eq:perplayer}; conditioning on tied conflict edges alone ($C_4$, grey, shifted for display) is not
affine.}
\label{fig:law-SM}
\end{figure}


Theorem~\ref{thm:pattern-SM} was also checked against exhaustive enumeration on $P_4$, $S_4$, $C_4$, $C_5$ and random
graphs with $N\le6$, $K\le5$ (Figure~\ref{fig:law-SM}). The full pattern is needed: on $C_4$, $P_4$ and $S_4$ ($K=3$,
averaged over all $24$ orders) the conditional energy equals $\calA_C(\tau)+\mathsf c_C$ to within $4\times10^{-10}$,
whereas conditioning on the number of tied conflict edges alone is not monotone on $C_4$.



\subsection{Randomised tie-breaking}
A deterministic protocol amplifies the harmonic component but does not create it.

\begin{propS}[randomised tie-breaking]\label{prop:randtie-SM}
If ties are broken uniformly at random and payoffs are taken in expectation, $\Epot$ is as in
Proposition~\ref{prop:energies} and $\Eharm$ is multiplied by $(K-2)/(K+1)$. The game is an exact potential game iff
$K=2$.
\end{propS}
\begin{proof}
Now $\psi(x,y)=-\frac12-\frac12\sgn(y-x)$ for every ordered pair, so again $\psi(x,y)+\psi(y,x)\equiv-1$,
$\omega^+\equiv0$, and the own effect is unchanged. Moreover $\Var\psi=\frac{K-1}{4K}$, so
$\|\omega\|^2=\frac{K-1}{4K}-\frac{K^2-1}{6K^2}=\frac{(K-1)(K-2)}{12K^2}$, which is $(K-2)/(K+1)$ times the deterministic
value $\frac{K^2-1}{12K^2}$ of Proposition~\ref{prop:energies}. Apply Proposition~\ref{prop:pairwise}(c),(d).
\end{proof}
What creates the harmonic component is the antisymmetry of the comparison, $\psi(x,y)+\psi(y,x)\equiv-1$; the
deterministic protocol adds to it the resolution of ties, which is why the factor vanishes at $K=2$, where every
randomly resolved tie is a coin flip with no residual interaction.

\section{The continuum game and the proof of Theorem~\ref{thm:spectrum}}\label{sec:cont}

\subsection{Setting}
Let $N$ players choose $s_i\in[0,1]$ i.i.d.\ uniformly,
$\pos_i(s)=\#\{j\ne i:s_j>s_i\}$ and $u_i=f(\pos_i)$. Flows are
functions $x_i(t\to t';s_{-i})$, antisymmetric in $(t,t')$, with
$\|x\|^2=\sum_i\E_{s_{-i}}\big[\frac12\iint x_i(t\to t';s_{-i})^2\,dt\,dt'\big]$;
gradients are $(\delta\phi)_i=\phi(t',s_{-i})-\phi(t,s_{-i})$, game
flows are $u_i(t',s_{-i})-u_i(t,s_{-i})$, and $P$ is the orthogonal
projection onto the closure of $\operatorname{im}\delta$. For
$v,w\in L^2([0,1]^N)$ one has
$\langle\delta_iv,\delta_iw\rangle_i=\E[(v-A_iv)(w-A_iw)]$ because
$\frac12\iint(v(t')-v(t))(w(t')-w(t))\,dt\,dt'=\Cov_{t}(v,w)$.

\begin{propS}[Hodge projection is the inverse number operator]\label{prop:Ninv}
With $g=\sum_i(u_i-A_iu_i)$, $Pu=\delta\phi^\star$ with
$\phi^\star=\numop^{-1}g$, and
\begin{equation}\label{eq:contP}
\|Pu\|^2=\sum_{m\ge1}\frac{\|g_m\|^2}m
=\sum_{T\ne\emptyset}\frac1{|T|}\Big\|\sum_{i\in T}[u_i]_T\Big\|^2,\qquad
\|u\|^2=\sum_i\|u_i-A_iu_i\|^2=\sum_i\sum_{T\ni i}\|[u_i]_T\|^2 .
\end{equation}
\end{propS}
\begin{proof}
$\|u-\delta\phi\|^2=\sum_i\|(I-A_i)(u_i-\phi)\|^2$ is minimised at the
solution of $\sum_i(I-A_i)\phi=\sum_i(I-A_i)u_i$, i.e.\ $\numop\phi=g$;
$\numop$ is invertible on mean-zero functions (it multiplies the order-$m$
component by~$m$), and
$\|\delta\phi^\star\|^2=\langle\numop\phi^\star,\phi^\star\rangle=\langle g,\numop^{-1}g\rangle$.
The second expression for $\|u\|^2$ is Parseval for the Hoeffding
decomposition, since $u_i-A_iu_i$ consists of the components with
$T\ni i$.
\end{proof}

\subsection{The two energies (\texorpdfstring{eq.~\eqref{eq:contquad}}{the two quadratic forms} of the main text)}

\begin{lemmaS}[Dirichlet variance identity]\label{lem:dir}
$\Var(u_i)=\Var_{k\sim U\{0,\dots,N-1\}}f(k)$ and
$\Var(\bar u_i)=\frac1{N+1}\Var(u_i)$; hence
$\|u\|^2=\frac{N^2}{N+1}\Var_kf(k)$.
\end{lemmaS}
\begin{proof}
$\pos_i$ is uniform on $\{0,\dots,N-1\}$ (positions form a uniformly
random permutation). Given $s_{-i}$ with order statistics
$z_1>\dots>z_{N-1}$ and spacings $\varsigma_k=z_k-z_{k+1}$ ($z_0=1$, $z_N=0$),
$\pos_i=k$ iff $z_{k+1}<s_i<z_k$, so $\bar u_i=\sum_kf(k)\varsigma_k$. The
spacings are Dirichlet$(1,\dots,1)$ with $N$ cells:
$\E\varsigma_k=\frac1N$, $\E\varsigma_k\varsigma_l=\frac{1+\delta_{kl}}{N(N+1)}$.
Hence $\E\bar u_i^2=\frac1{N(N+1)}\big[(\sum_kf_k)^2+\sum_kf_k^2\big]$ and
$\Var\bar u_i=\frac1{N+1}\big[\frac1N\sum f_k^2-\frac1{N^2}(\sum f_k)^2\big]
=\frac1{N+1}\Var_kf$. Finally
$\|u\|^2=\sum_i[\Var u_i-\Var\bar u_i]=N\cdot\frac{N}{N+1}\Var_kf$.
\end{proof}

\begin{lemmaS}[Bernoulli-sum decomposition]\label{lem:bern}
Let $B_t=\#\{j\ne i:s_j>t\}$ and $\kappa(t,t')=\min(t,t')-tt'$. For
$T\not\ni i$ with $|T|=m$,
\[
[\bar u_i]_T=\int_0^1\prod_{j\in T}\big(\one[s_j>t]-(1-t)\big)\,d_m[f](1-t)\,dt,\qquad
d_m[f](q)=\E\big[\Delta^mf(\Bin(N-1-m,q))\big],
\]
and this expression does not depend on $i\notin T$. Consequently
\begin{equation}\label{eq:gmJm}
\|g_m\|^2=(N-m)^2J_m,\qquad
J_m:=\binom Nm\iint\kappa(q,q')^m\,d_m[f](q)\,d_m[f](q')\,dq\,dq',
\end{equation}
and $\|Pu\|^2=\sum_m\frac{(N-m)^2}mJ_m$, $\|u\|^2=N\sum_m(N-m)J_m$.
\end{lemmaS}
\begin{proof}
$\bar u_i(s_{-i})=\int_0^1f(B_t)\,dt$, since $\pos_i=B_{s_i}$ and $s_i$ is
uniform. For fixed $t$, $B_t$ is a sum of i.i.d.\ Bernoulli$(1-t)$
variables $\xi_j=\one[s_j>t]$; for a function $F$ of such a sum, the
Hoeffding component on $T$ is
$\prod_{j\in T}(\xi_j-(1-t))\cdot\E[\Delta^{|T|}F(B^{(T^c)}_t)]$
(expand $F(\xi_T+B^{(T^c)})$ in the Walsh basis
$\prod_{j\in T}(\xi_j-(1-t))$; each centred factor acts as a forward
difference). Integrating over $t$ gives the formula, whose right-hand
side involves $i$ only through the size $N-1-m$ of the complement.
By Lemma~\ref{lem:cons}, $g_T=-\sum_{i\notin T}[\bar u_i]_T=-(N-m)\times$ the
common expression; its squared norm is computed using
$\E\big[(\one[s>t]-(1-t))(\one[s>t']-(1-t'))\big]=\kappa(t,t')$ for each of
the $m$ coordinates, which gives \eqref{eq:gmJm} after the substitution
$q=1-t$, under which $\kappa$ is invariant. The formula for
$\|Pu\|^2$ is \eqref{eq:contP}. For $\|u\|^2$: the same computation gives
$\Var(\bar u_i)=\sum_m\binom{N-1}m\iint\kappa^md_md_m$, and Lemma~\ref{lem:dir}
yields $\|u\|^2=N\big[\Var u_i-\Var\bar u_i\big]=N^2\Var\bar u_i
=N^2\sum_m\binom{N-1}m\iint\kappa^md_md_m=N\sum_m(N-m)J_m$, using
$N\binom{N-1}m=(N-m)\binom Nm$.
\end{proof}

\begin{proof}[Proof of Corollary~\ref{cor:Qinf}, with the equality case]
Since $\rho^{(\infty)}_\pot(f)=\|Pu\|^2/\|u\|^2$, it suffices to show that, by Lemma~\ref{lem:bern},
\[
\frac{N-1}N\|u\|^2-\|Pu\|^2=\sum_m(N-m)J_m\Big[(N-1)-\frac{N-m}m\Big]
=\sum_{m\ge1}(N-m)J_m\frac{N(m-1)}m\ \ge0,
\]
since $J_m\ge0$ ($\kappa^m$ is a positive semidefinite kernel). Equality holds iff $J_m=0$ for all
$m\ge2$, i.e.\ $d_m[f]\equiv0$; as $q\mapsto\E[\Delta^mf(\Bin(n,q))]$ is the
Bernstein polynomial of $\Delta^mf$, this holds iff $\Delta^mf\equiv0$
for all $m\ge2$, i.e.\ iff $f$ is affine.
\end{proof}

\subsection{Proof of Theorem~\ref{thm:spectrum}}

\begin{mainthm}[\ref{thm:spectrum} of the main text]
Let $t_p(k)=\sum_{r=0}^p(-1)^r\binom pr\binom{p+r}r\frac{\ff kr}{\ff{(N-1)}r}$, $p=1,\dots,N-1$, be the discrete
Chebyshev polynomials, and $J_m(f,g)=\binom Nm\iint\kappa^m\,d_m[f](q)\,d_m[g](q')\,dq\,dq'$ the order-$m$ form, so that
$\mathcal E_\pot(f,g):=\sum_m\frac{(N-m)^2}mJ_m(f,g)$ and $\mathcal E_{\rm tot}(f,g):=N\sum_m(N-m)J_m(f,g)$ polarise
$\|Pu\|^2$ and $\|u\|^2$.
\begin{enumerate}
\item[(a)] For every $m$ and all $p\ne p'$, $J_m(t_p,t_{p'})=0$; moreover $J_m(t_p,t_p)=0$ for $m>p$ and, for $m\le p$,
\begin{equation}\label{eq:JdiagS}
J_m(t_p,t_p)=\binom Nm\frac{m\,(p+m)!}{p(p+1)(2p+1)\,(p-m)!\,\big[\ff{(N-1)}m\big]^2}.
\end{equation}
\item[(b)] $\displaystyle\lambda_p=\frac{\mathcal E_\pot(t_p,t_p)}{\mathcal E_{\rm tot}(t_p,t_p)}
=\frac{(N-p)(N+p+1)}{N\,p(p+1)}\Big[1-\frac{\binom Np}{\binom{N+p+1}p}\Big]$, and $\lambda_{p+1}<\lambda_p$ for
$1\le p\le N-2$.
\end{enumerate}
\end{mainthm}
Throughout, $q=1-t$, $\kappa=\min(q,q')-qq'$ and $d_m[f](q)=\E[\Delta^mf(\Bin(N-1-m,q))]$ as in Lemma~\ref{lem:bern};
$n:=N-1$; $\tilde P_p(q):=P_p(1-2q)=\sum_{r=0}^p(-1)^r\binom pr\binom{p+r}r q^r$ is the shifted Legendre polynomial,
$\tilde P^{(m)}_j(q):=P^{(m,m)}_j(1-2q)$ the shifted Jacobi (Gegenbauer) polynomial, and $\mathsf w_m(q):=[q(1-q)]^m$.

\paragraph{(i) From Chebyshev to Legendre and Jacobi polynomials.}
Let $\mathsf b_f(q):=\E f(\Bin(n,q))$ be the Bernstein polynomial of $f$. For $f=\ff kr$ one has
$\E[\ff{\Bin(n,q)}r]=\ff nr\,q^r$ and $\Delta^m\ff kr=\ff rm\,\ff k{r-m}$, hence
$d_m[\ff kr](q)=\ff rm\,\ff{(n-m)}{r-m}\,q^{r-m}=\frac1{\ff nm}\frac{d^m}{dq^m}\big(\ff nr\,q^r\big)$, because
$\ff nr=\ff nm\,\ff{(n-m)}{r-m}$. By linearity,
\begin{equation}\label{eq:bernder}
d_m[f]=\frac{1}{\ff nm}\,\mathsf b_f^{(m)}\qquad\text{for every }f,
\end{equation}
which is the classical derivative formula for Bernstein polynomials. Moreover
$\mathsf b_{t_p}(q)=\sum_r(-1)^r\binom pr\binom{p+r}rq^r=\tilde P_p(q)$: the binomial law maps the discrete Chebyshev
polynomials to the Legendre polynomials. Since $\frac{d^m}{dx^m}P_p(x)=\frac{(p+m)!}{2^m\,p!}P^{(m,m)}_{p-m}(x)$ and
$\frac d{dq}=-2\frac d{dx}$ for $x=1-2q$,
\begin{equation}\label{eq:dmtp}
d_m[t_p](q)=c_{p,m}\,\tilde P^{(m)}_{p-m}(q),\qquad c_{p,m}:=\frac{(-1)^m(p+m)!}{p!\,\ff nm}\quad(m\le p),
\end{equation}
and $d_m[t_p]=0$ for $m>p$.

\paragraph{(ii) The kernel $\kappa^m$ carries the Jacobi weight.}
Let $\mathsf K_mg(q):=\int_0^1\kappa(q,q')^mg(q')\,dq'$.
\begin{lemmaS}\label{lem:Km}
{\rm(a)} If $g$ is a polynomial of degree at most $b$, then $\mathsf K_mg=\mathsf w_m\,R$ with $R$ a polynomial of
degree at most $b$. {\rm(b)} For every $j\ge0$,
\[
\mathsf K_m\tilde P^{(m)}_j=\mathsf k_{m,j}\,\mathsf w_m\,\tilde P^{(m)}_j,\qquad\mathsf k_{m,j}=\frac{m}{(j+m)(j+m+1)} .
\]
\end{lemmaS}
\begin{proof}
(a) It suffices to take $g=q^b$. Since $\kappa(q,s)=s(1-q)$ for $s\le q$ and $q(1-s)$ for $s\ge q$,
\[
\mathsf K_mg(q)=(1-q)^m\frac{q^{m+b+1}}{m+b+1}+q^m\,G(q),\qquad G(q):=\int_q^1(1-s)^ms^b\,ds .
\]
$G$ is a polynomial of degree $m+b+1$ with $G^{(i)}(1)=0$ for $i\le m$, so $G=(1-q)^{m+1}G_1$ with $\deg G_1=b$; the
leading coefficient of $G$ is $-(-1)^m/(m+b+1)$, hence that of $G_1$ is $1/(m+b+1)$. Thus
$\mathsf K_mg=\mathsf w_m\big[\frac{q^{b+1}}{m+b+1}+(1-q)G_1\big]$, and in the bracket the coefficients of $q^{b+1}$
cancel.

(b) $\mathsf K_m$ is self-adjoint on $L^2(0,1)$. Write $\mathsf K_m\tilde P^{(m)}_j=\mathsf w_mR$ with $\deg R\le j$. For
a polynomial $S$ of degree $<j$, part (a) gives $\mathsf K_mS=\mathsf w_mR_S$ with $\deg R_S<j$, so
$\int S\,\mathsf w_m R=\int(\mathsf K_mS)\tilde P^{(m)}_j=\int\mathsf w_mR_S\,\tilde P^{(m)}_j=0$, because the
$\tilde P^{(m)}_j$ are orthogonal for the weight $\mathsf w_m$. Hence $R$ is orthogonal, for that weight, to all
polynomials of lower degree, i.e.\ $R=\mathsf k\,\tilde P^{(m)}_j$. To find $\mathsf k$ let $q\to0$: the first term of the
display above is $O(q^{m+1})$, so
$\mathsf K_m\tilde P^{(m)}_j(q)=q^m\int_0^1(1-s)^m\tilde P^{(m)}_j(s)\,ds+O(q^{m+1})$, while
$\mathsf w_m\tilde P^{(m)}_j=q^m\tilde P^{(m)}_j(0)+O(q^{m+1})$ with $\tilde P^{(m)}_j(0)=P^{(m,m)}_j(1)=\binom{j+m}j$.
The Rodrigues formula reads $\mathsf w_m\tilde P^{(m)}_j=\frac1{j!}\frac{d^j}{ds^j}\big[s^{j+m}(1-s)^{j+m}\big]$, and
$j$ integrations by parts (all boundary terms vanish) give
\begin{align*}
\int_0^1(1-s)^m\tilde P^{(m)}_j\,ds&=\frac1{j!}\int_0^1s^{-m}\frac{d^j}{ds^j}\big[s^{j+m}(1-s)^{j+m}\big]ds\\
&=\frac{m(m+1)\cdots(m+j-1)}{j!}\int_0^1(1-s)^{j+m}ds=\frac{\binom{m+j-1}j}{j+m+1}.
\end{align*}
Dividing by $\binom{j+m}j$ gives $\mathsf k_{m,j}=\frac{m}{(j+m)(j+m+1)}$.
\end{proof}

\paragraph{(iii) Every order form is diagonal; the potential form.}
By \eqref{eq:dmtp} and Lemma~\ref{lem:Km}(b), for $m\le\min(p,p')$,
\[
J_m(t_p,t_{p'})=\binom Nm c_{p,m}c_{p',m}\,\mathsf k_{m,p'-m}\int_0^1\mathsf w_m\,\tilde P^{(m)}_{p-m}\tilde P^{(m)}_{p'-m}\,dq,
\]
which vanishes for $p\ne p'$ by Jacobi orthogonality; this is (a), the case $m>\min(p,p')$ being trivial. For $p=p'$,
$\mathsf k_{m,p-m}=\frac m{p(p+1)}$ and the Jacobi norm
$\int_0^1\mathsf w_m\big(\tilde P^{(m)}_{p-m}\big)^2dq=\frac{(p!)^2}{(2p+1)\,(p+m)!\,(p-m)!}$ give \eqref{eq:JdiagS}.
In particular the $t_p$ diagonalise $\sum_mw_mJ_m$ for any weights $w_m$, hence both $\mathcal E_\pot$ and
$\mathcal E_{\rm tot}$ (for the latter this is also clear from
$\mathcal E_{\rm tot}(f,f')=\frac N{N+1}\sum_k(f_k-\bar f)(f'_k-\bar f')$, Lemma~\ref{lem:dir}). Finally, with
$\binom Nm(N-m)^2/[\ff nm]^2=N\,(N-m)!/[m!\,(N-1)!]$,
\[
\mathcal E_\pot(t_p,t_p)=\sum_{m=1}^p\frac{(N-m)^2}mJ_m(t_p,t_p)
=\frac{N}{(N-1)!\,p(p+1)(2p+1)}\sum_{m=1}^p\frac{(N-m)!\,(p+m)!}{m!\,(p-m)!}.
\]
In the same way $N(N-m)J_m(t_p,t_p)\propto(N-m-1)!\,(p+m)!/[(m-1)!\,(p-m)!]$, which is the distribution $\eta_{p,m}$ of
the energy of $t_p$ over the orders quoted in the main text.

\paragraph{(iv) Normalisation and closed form.}
The Hahn-polynomial norm (parameters $(0,0)$) gives
$\sum_{k=0}^{N-1}t_p(k)^2=\frac{(N+p)!\,(N-1-p)!}{(2p+1)\,(N-1)!^2}$, so
$\mathcal E_{\rm tot}(t_p,t_p)=\frac N{N+1}\cdot\frac{(N+p)!(N-1-p)!}{(2p+1)(N-1)!^2}$ and
\[
\lambda_p=\frac{(N+1)!}{N\,p(p+1)\,(N-p-1)!\,(N+p)!}\sum_{m=1}^p\frac{(p+m)!\,(N-m)!}{m!\,(p-m)!}.
\]
Adding the $m=0$ term $N!$, the sum becomes
\[
N!\;{}_2F_1(-p,\,p+1;\,-N;\,1)=\frac{(N+p+1)!\,(N-p)!}{(N+1)!}
\]
by the Chu--Vandermonde identity,\footnote{The lower parameter $-N$ is a
nonpositive integer, so ${}_2F_1$ is meant here as the terminating series
determined by the upper parameter $-p$. This is legitimate: the series
stops after $p+1\le N$ terms, and $(-N)_m\ne0$ for $0\le m\le p\le N-1$,
so every term is finite. Chu--Vandermonde in the form
${}_2F_1(-p,b;c;1)=\frac{(c-b)_p}{(c)_p}$ is an identity between rational
functions of $c$, and $(c)_p$ does not vanish at $c=-N$ when $p\le N$; it
may therefore be evaluated at $c=-N$. Explicitly,
$(-N)_p=(-1)^p\frac{N!}{(N-p)!}$ and $(-N-p-1)_p=(-1)^p\frac{(N+p+1)!}{(N+1)!}$.}
which yields the stated closed form
with
\[
\varepsilon_p:=\frac{\binom Np}{\binom{N+p+1}p}=\prod_{i=0}^{p-1}\frac{N-i}{N+p+1-i}.
\]
For $p=1$, $\varepsilon_1=\frac N{N+2}$ and $\lambda_1=\frac{N-1}N$.

\paragraph{(v) Monotonicity.}
Put $D_p=\frac{N(N+1)}{p(p+1)}-1$, so $N\lambda_p=D_p(1-\varepsilon_p)$,
$D_p-D_{p+1}=\frac{2N(N+1)}{p(p+1)(p+2)}$ and
$\varepsilon_{p+1}=\varepsilon_p\frac{N-p}{N+p+2}$. Then $\lambda_p>\lambda_{p+1}$ reads
$D_p(1-\varepsilon_p)>D_{p+1}\big(1-\varepsilon_p\frac{N-p}{N+p+2}\big)$; since
$D_p-D_{p+1}\frac{N-p}{N+p+2}=(D_p-D_{p+1})+D_{p+1}\frac{2(p+1)}{N+p+2}$, this is
$(D_p-D_{p+1})(1-\varepsilon_p)>\varepsilon_p\,D_{p+1}\frac{2(p+1)}{N+p+2}$, i.e., with
$D_{p+1}=\frac{(N-p-1)(N+p+2)}{(p+1)(p+2)}$,
\[
\frac{1-\varepsilon_p}{\varepsilon_p}>\frac{2(p+1)D_{p+1}}{(D_p-D_{p+1})(N+p+2)}=\frac{p(p+1)(N-p-1)}{N(N+1)} .
\]
Now $\varepsilon_p^{-1}=\prod_{i=0}^{p-1}\frac{N+p+1-i}{N-i}=\prod_{i=0}^{p-1}\Big(1+\frac{p+1}{N-i}\Big)\ge1+\frac{p(p+1)}N$,
so the left-hand side is at least $\frac{p(p+1)}N$, which exceeds the right-hand side because $N-p-1<N+1$. \qed

\begin{remarkS}
Every step is audited in exact arithmetic by \texttt{audits/check\_spectrum.py} (\eqref{eq:bernder}, \eqref{eq:dmtp},
Lemma~\ref{lem:Km}, \eqref{eq:JdiagS} against direct evaluation of the double integrals, and the closed forms of
$\lambda_p$ and of the total form for $3\le N\le9$). Part (i) is the mechanism behind the appearance of the same
polynomials and of $\varepsilon_p$ in the spectra of the Beta--binomial Gibbs sampler and the Bernstein--Durrmeyer
operators cited in the main text.
\end{remarkS}

\section{Priced priorities}\label{sec:priced}
This appendix proves the statement made after Corollary~\ref{cor:rigid} of the main text: pricing can change
behaviour drastically while leaving $\Eharm$ fixed, and neither energy predicts the existence of pure equilibria. The
protocol is the index protocol and $C$ is an arbitrary conflict graph.

\begin{propS}[priced priorities]\label{prop:priced-SM}
Let $u_i(s)=-\pos_C(i,s)-c\,s_i$ with $c>0$, and $b_i:=\#\{j\in\calN(i):j<i\}$.
\begin{enumerate}
\item[(a)] $\Eharm$ is as in Proposition~\ref{prop:energies} and $\Epot=c_K\sum_i(d_i-cK)^2$. On a $d$-regular graph
the game is purely harmonic at $c=d/K$, where marginal price equals marginal expected benefit, and uniform mixing is
then a Nash equilibrium.
\item[(b)] If $0<c<1$ and $E\neq\emptyset$, there is no pure Nash equilibrium.
\item[(c)] The all-zero profile is a Nash equilibrium iff $c\ge\max_ib_i$.
\end{enumerate}
\end{propS}
\begin{proof}
(a) Pricing replaces the own effect $\mathsf a_i(x)=d_i(x-\bar s)/K$ of Proposition~\ref{prop:energies} by
$(d_i/K-c)(x-\bar s)$ and nothing else; apply Proposition~\ref{prop:pairwise}(c). If all other agents mix uniformly,
$\E[u_i\mid s_i=x]=\mathrm{const}+x(d_i/K-c)$, constant in $x$ at $c=d/K$.

(b) Let $s$ be a pure equilibrium. For an agent with $s_i\ge1$ let $L_i\in\mathbb{Z}_{\ge0}$ be the number of positions
lost by lowering one level; no profitable deviation means $L_i\ge c>0$, so $L_i\ge1$. For an agent with $s_i\le K-2$
let $W_i$ be the number of neighbours overtaken by raising one level; then $W_i\le c<1$, so $W_i=0$. In particular
isolated agents sit at level $0$. If all agents are at level $0$, take an edge $\{i,j\}$ with $i<j$: raising $j$ to
level $1$ overtakes $i$, so $W_j\ge1$, a contradiction. Otherwise let $s_{\max}\ge1$ be the highest occupied level and
$m$ the largest-index agent at it. Since $L_m\ge1$, some neighbour $j$ is served before $m$ after $m$ lowers but not
before; this requires either $s_j=s_{\max}$ with $j>m$, excluded by the choice of $m$, or $s_j=s_{\max}-1$ with $j<m$.
In the latter case $j$, raising one level, ties $m$ and is favoured by the protocol, so $W_j\ge1$, a contradiction.

(c) At $s=0$ every agent is tied with all neighbours, so $u_i=-b_i$. Raising to level $t\ge1$ puts $i$ ahead of every
neighbour at payoff $-ct$, best at $t=1$. The deviation is strictly profitable iff $c<b_i$.
\end{proof}

Thus pure equilibria exist at $c=0$, vanish on all of $(0,1)$, and reappear for larger $c$, while $\Eharm$ does not
move. Part~(b) uses the index protocol: on a triangle with the cyclic protocol and $K=2$, the profile in which everybody
bids $1$ is an equilibrium for every $c<1$.

\paragraph{Exact computation on the intersection.} Scanning $c$ over $91$ values in $[0,4.5]$ on the eight-vehicle
intersection ($K=3$), with the methods of Section~\ref{sec:numerics} of the main text, the potential share follows
(a) to machine precision, from $4/5$ at $c=0$ through exactly $0$ at $c=d/K=4/3$ back to $0.96$ at $c=4.5$, while
the projected harmonic energy is constant to $10^{-14}$ and the entropy production at $\beta\max|\Delta u|=0.02$ stays
within $3\times10^{-5}$ of the prediction of Proposition~\ref{prop:learning}. Pure equilibria number three at $c=0$,
zero on $(0,1)$ as in (b), and one from $c=\max_ib_i=4$ on as in (c); in between they exist only at $c=1$ and $c=3$,
a feature of this graph (a star whose centre has the largest index has one for every $c\in(1,\max_ib_i)$).



\section{Reproducibility and independent audit}\label{app:repro}
The proof of Theorem~\ref{thm:finiteK} is computer-assisted at three places only---the root isolation of
Step~\ref{step:K4}, the symbolic identities in $N$ of Step~\ref{step:K3}, and the certificates of
Step~\ref{step:certs}---and every other step, and all of Appendices~\ref{sec:pattern}--\ref{sec:priced}, is proved by
hand. Table~\ref{tab:scripts} lists the scripts of those three steps; they use exact arithmetic only (Python
\texttt{fractions} or SymPy), and \texttt{run\_checks.sh} runs them all in well under a minute. The floating-point
computations of Section~\ref{sec:numerics} of the main text and of Appendix~\ref{sec:priced} enter no proof and are
kept outside the package.

\begin{table}[H]\centering\small
\caption{Scripts on which the proof of Theorem~\ref{thm:finiteK} depends, and the two independent checks.}\label{tab:scripts}
\begin{tabular}{@{}>{\raggedright\arraybackslash}p{0.33\linewidth}>{\raggedright\arraybackslash}p{0.09\linewidth}>{\raggedright\arraybackslash}p{0.52\linewidth}@{}}\toprule
script & step & establishes\\\midrule
\texttt{verify\_certificates.py} + \texttt{certificates/} ($25$ files) & \ref{step:certs} & the pairs of Table~\ref{tab:cov}: rebuilds each certified matrix from Theorem~\ref{thm:SOS} and Step~\ref{step:bond}, checks $LDL^\top=A$ with positive pivots and the kernel; standard library only, imports nothing\\
\texttt{audit\_K4.py} & \ref{step:K4} & the cubic of Lemma~\ref{lem:K4root}, exact root counting for $\varrho\ge\varrho_0$, and (T) for all bonds iff $N\ge10$ (Theorem~\ref{thm:K4}); also audits the hand-proved closed forms of Steps~\ref{step:Sqlow}--\ref{step:perron}\\
\texttt{k3\_representation\_proof.py}, \texttt{s1\_closed.py}, \texttt{check\_blocks.py}, \texttt{verify\_M\_symbolic.py} & \ref{step:K3} & Lemmas~\ref{lem:K3rep}, \ref{lem:K3blocks} and~\ref{lem:K3M}: the block representation, the closed forms of its entries, the row sums $\mathsf M\one$, and the certificates for $N=17,18$\\
\texttt{k2\_witness.py} & \ref{step:assembly} & the $K=2$, $N=7$ witness from the definition of the Hodge projection; $Q_2\one=0$; the sign change between $N=6$ and $N=7$\\
\texttt{end\_to\_end.py} & --- & Theorem~\ref{thm:finiteK} for $K=3$, $N\le7$; $K=4$, $N\le5$; $K=5$, $N\le4$; $K=6,7$, $N=3$, using no step of the proof (see below)\\\bottomrule
\end{tabular}
\end{table}

\paragraph{An end-to-end check that bypasses the proof.} \texttt{end\_to\_end.py} builds
$Q_K=\frac{N-1}NM_{\rm tot}-M_\pot$ directly from \eqref{eq:rayleigh}---all $K^N$ profiles, the flow of every
increment indicator, $M_\pot$ from the Hoeffding decomposition of the divergence (Lemma~\ref{lem:lap})---in exact
rational arithmetic, and certifies $Q_K\one=0$ and $Q_K+\one\one^\top=LDL^\top$ with positive pivots. This is
Theorem~\ref{thm:finiteK} for that pair, obtained without the order decomposition, the bond variables or the
sum-of-squares identity; it is feasible while $K^N$ is a few thousand, and at $K=2$ it reports positivity for $N\le6$
and failure at $N=7$. Any other pair: \texttt{python3 end\_to\_end.py K,N}. The package also contains the certificate
generator (\texttt{bond\_certificate.py}, \texttt{full\_space\_certificate.py}, \texttt{make\_certificates.py}), which
the checker does not import, and \texttt{audits/check\_spectrum.py}, a symbolic audit of the hand proof of
Theorem~\ref{thm:spectrum}.
